An Algebraic Study of Bilattice-based Logics

The aim of this work is to develop a study from the perspective of Abstract Algebraic Logic of some bilattice-based logical systems introduced in the nineties by Ofer Arieli and Arnon Avron. The motivation for such an investigation has two main roots. On the one hand there is an interest in bilattices as an elegant formalism that gave rise in the last two decades to a variety of applications, especially in the field of Theoretical Computer Science and Artificial Intelligence. In this respect, the present study aims to be a contribution to a better understanding of the mathematical and logical framework that underlie these applications. On the other hand, our interest in bilattice-based logics comes from Abstract Algebraic Logic. In very general terms, algebraic logic can be described as the study of the connections between algebra and logic. One of the main reasons that motivate this study is the possibility to treat logical problems with algebraic methods and viceversa: this is accomplished by associating to a logical system a class of algebraic models that can be regarded as the algebraic counterpart of that logic. Starting from the work of Tarski and his collaborators, the method of algebraizing logics has been increasingly developed and generalized. In the last two decades, algebraic logicians have focused their attention on the process of algebraization itself: this kind of investigation forms now a subfield of algebraic logic known as Abstract Algebraic Logic (which we abbreviate AAL).

==> Ch_2_Int__Pre_bilattices.tex <==
%\documentclass[a4paper, 11pt]{amsart}
%\usepackage{amsmath, amssymb, amsthm, enumerate, graphicx, pdfsync
%}
%\usepackage[notref,notcite]{showkeys} 
%\author{U. Rivieccio}
%\title{Chapter 2 \\ Interlaced (Pre-)Bilattices}
%\date{}
%\setlength{\textwidth}{415pt}
%\setlength{\oddsidemargin}{20pt}

%\input{preamble}

%\begin{document}

%\maketitle
%\tableofcontents 

%
%%\texttt{Veo que no pones en cursiva los enunciados de las proposiciones. He mirado el preamble y veo que usas 
%%siempre el estilo definition. Lo habitual es usar el estilo definition (que da tipografia normal) para definiciones, remarks y ejemplos, y el estilo theorem para teoremas, proposiciones y lemas. Si es que te gusta mas como lo has hecho continua con tu estilo.}

\chapter{Interlaced (pre-)bilattices} %2
\label{ch:int}

\section{Representation Theorem for pre-bilattices}
\label{sec:reppre}

In this section we generalize %[the result of] 
the Representation Theorem \ref{thm:reprpre} to the case of unbounded pre-bilattices. As noted in Chapter %1
\ref{ch:intro}, the proofs known in the literature use the bounds of the pre-bilattice to make a projection of sorts: this strategy leads to a decomposition  into two sub-pre-bilattices which, as we have noted, can also be seen simply as lattices. Our strategy, instead, will be to define two congruences on the pre-bilattice: the factors of our decomposition will then be obtained as quotients of the pre-bilattice modulo these two congruences.  



We start with some lemmas that are needed in the proof of the theorem and will help to understand better the structure of interlaced pre-bilattices.

First of all, let us note that there is a duality
implicit in the definition of $\IPBL$, which will help us to simplify
many of our proofs.
\begin{rem}[Duality Principle]
Let  $\Al[B] = \langle B, \leq_t, \leq_k  \rangle$ be a pre-bilattice and let $\leq_t^{\partial}$ and $\leq_k^{\partial}$ denote the dual orders of $\leq_t$ and $\leq_k$ respectively.  A \emph{dual algebra} of  $\Al[B]$ is any of the pre-bilattices $\la B, \leq_t^{\partial}, \leq_k\ra,$  $\la B, \leq_t^{\partial}, \leq_k^{\partial}\ra$ and
$\la B, \leq_t, \leq_k^{\partial}\ra$. It is easy to see that the class $\IPBL$ is closed under
  dual algebras: hence any property that holds in all
  the members of $\IPBL$ also holds in any dual
  algebra of an interlaced pre-bilattice.
\end{rem}

%\texttt{Tal como das la definici\'on, $\Al[B]$ es dual de $\Al[B]$ y $\la B, \wedge, \vee, \wedge, \vee\ra$ tambi\'en. Parece raro. No se ajusta a lo que uno espera al leer "dual". Creo que es mejor utilizar los ordenes en lugar de las operaciones para decir lo que quieres decir.  Yo diria:\\
%A \emph{dual algebra} of  $\Al[B]$ is any of the pre-bilattices $\la B, \leq_t^{\partial}, \leq_k\ra,  \la B, \leq_t^{\partial}, \leq_k^{\partial}\ra,\\
%\la B, \leq_t, \leq_k^{\partial}\ra$.
%$^{\partial}$ significa dual}

Given two orderings $\leq_1$ and $\leq_2$ defined on the same set, we denote by $\leq_1 \circ \leq_2$ the usual composition of the two relations. Thus, $\langle a,b \rangle \in \: \leq_1 \circ \leq_2$ means that there is some $c$ such that $a \leq_1 c \leq_2 b$. We can now state the following:

%\begin{proposition} \label{fileq2}
%Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus \rangle$ be an interlaced pre-bilattice and $a, b \in B$. The following are equivalent:

%\begin{align*}
%\textrm{(i)} \quad & a \leq_k a \land b  & \textrm{(v)} \quad & \langle a,b \rangle \in \: \leq_k \circ \leq_t \\
%  \textrm{(ii)} \quad & a \leq_t a \otimes b    & \textrm{(vi)} \quad & \langle a,b \rangle \in \: \leq_t \circ \leq_k \ \\
% \textrm{(iii)} \quad &  a \lor b \leq_k b & \textrm{(vii)} \quad &  \langle b,a \rangle \in \: \geq_k \circ \geq_t  \\
% \textrm{(iv)} \quad & a \oplus b \leq_t b    & \textrm{(viii)} \quad & \langle b,a \rangle \in \: \geq_t \circ \geq_k.
%\end{align*}
%\end{proposition}
%
%\begin{align*}
%\textrm{(i)} \quad & a \leq_k a \land b  & \textrm{(v)} \quad & \langle a,b \rangle \in \: \leq_k \circ \leq_t \\
%  \textrm{(ii)} \quad & a \leq_t a \otimes b    & \textrm{(vi)} \quad & \langle a,b \rangle \in \: \leq_t \circ \leq_k \ \\
% \textrm{(iii)} \quad &  a \lor b \leq_k b & \textrm{(vii)} \quad &  \langle b,a \rangle \in \: \geq_k \circ \geq_t  \\
% \textrm{(iv)} \quad & a \oplus b \leq_t b    & \textrm{(viii)} \quad & \langle b,a \rangle \in \: \geq_t \circ \geq_k.
%\end{align*}


%\texttt{La proposici\'on es dif\'icil de leer. Mira si se te ocurre una forma mas clara visualmente}

%\texttt{Umberto: He intentado mejorar la proposicion 1.2: espero que ahora se lea mejor.}


\begin{proposition} \label{fileq}
Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus \rangle$ be an interlaced pre-bilattice. Then, for all $a, b \in B:$

\begin{tabular}[c]{lllllllllllll}
\\
(i) &&&& $a \leq_k a \land b$      &&& $\Leftrightarrow$ &&& $\langle a,b \rangle \in \: \leq_k \circ \leq_t$    && $\Leftrightarrow$ \\
    &&&& $a \leq_t a \otimes b$   &&& $\Leftrightarrow$ &&& $\langle a,b \rangle \in \: \leq_t \circ \leq_k $    && $\Leftrightarrow$ \\ 
    &&&& $a \lor b \leq_k b   $      &&& $\Leftrightarrow$ &&& $\langle b,a \rangle \in \: \geq_k \circ \geq_t$  && $\Leftrightarrow$  \\
    &&&& $a \oplus b \leq_t b$     &&& $\Leftrightarrow$ &&& $\langle b,a \rangle \in \: \geq_t \circ \geq_{k.}  $ \\ \\
(ii) &&&& $a \leq_k a \lor b$      &&& $\Leftrightarrow$ &&& $\langle a,b \rangle \in \: \leq_k \circ \geq_t$    && $\Leftrightarrow$ \\
    &&&& $a \geq_t a \otimes b$   &&& $\Leftrightarrow$ &&& $\langle a,b \rangle \in \: \geq_t \circ \leq_k $    && $\Leftrightarrow$ \\ 
    &&&& $a \land b \leq_k b   $      &&& $\Leftrightarrow$ &&& $\langle b,a \rangle \in \: \geq_k \circ \leq_t$  && $\Leftrightarrow$  \\
    &&&& $a \oplus b \geq_t b$     &&& $\Leftrightarrow$ &&& $\langle b,a \rangle \in \: \leq_t \circ \geq_{k.}  $ \\ \\
    (iii) &&&& $a \geq_k a \land b$     &&& $\Leftrightarrow$ &&& $\langle a,b \rangle \in \: \geq_k \circ \leq_t$    && $\Leftrightarrow$ \\
    &&&& $a \leq_t a \oplus b$   &&& $\Leftrightarrow$ &&& $\langle a,b \rangle \in \: \leq_t \circ \geq_k $    && $\Leftrightarrow$ \\ 
    &&&& $a \lor b \geq_k b   $      &&& $\Leftrightarrow$ &&& $\langle b,a \rangle \in \: \leq_k \circ \geq_t$  && $\Leftrightarrow$  \\
    &&&& $a \otimes b \leq_t b$     &&& $\Leftrightarrow$ &&& $\langle b,a \rangle \in \: \geq_t \circ \leq_{k.}  $ \\ \\
    (iv) &&&& $a \geq_k a \lor b$      &&& $\Leftrightarrow$ &&& $\langle a,b \rangle \in \: \geq_k \circ \geq_t$    && $\Leftrightarrow$ \\
    &&&& $a \geq_t a \oplus b$   &&& $\Leftrightarrow$ &&& $\langle a,b \rangle \in \: \geq_t \circ \geq_k $    && $\Leftrightarrow$ \\ 
    &&&& $a \land b \geq_k b   $      &&& $\Leftrightarrow$ &&& $\langle b,a \rangle \in \: \leq_k \circ \leq_t$  && $\Leftrightarrow$  \\
    &&&& $a \otimes b \geq_t b$     &&& $\Leftrightarrow$ &&& $\langle b,a \rangle \in \: \leq_t \circ \leq_{k.}  $ \\
\end{tabular} 
\end{proposition}

\begin{proof}
  By the Duality Principle, it is enough to prove (i). Indeed, it is enough to prove the equivalence among the first four properties of (i), since the remaining four 
  correspond to the first four properties of (iv) just permuting $a$
  and $b$. Let us denote by (1), (2), (3) and (4) each one of
  the first four claims of (i).

(1) $\Rightarrow$ (2): If $a \leq_k a \land b$, then it is obvious that
$a \leq_k a \land b \leq_t b$. Therefore, $\langle a,b \rangle \in \:
\leq_k \circ \leq_t$.

(2) $\Rightarrow$ (3): Let us assume that there is some $c$ such that
$a \leq_k c \leq_t b$. Then, by the interlacing conditions we have $a = a
\otimes c \leq_t a \otimes b$.

(3) $\Rightarrow$ (4): If $a \leq_t a \otimes b$, then $a \leq_t a
\otimes b \leq_k b$. Thus, $\langle a,b \rangle \in \: \leq_t \circ
\leq_k$.

(4) $\Rightarrow$ (1): If $a \leq_t c \leq_k b$ for some $c$, then by
the interlacing conditions it holds that $a = a \land c \leq_k a \land b$.
\end{proof}



\begin{cor} 
  \label{cor:interlacingorders}
Let $\Al[B]$ be an interlaced pre-bilattice. Then, for every $\leq_1, \leq_2
\: \in \{ \leq_t, \geq_t,$ $\leq_k, \geq_k \}$ it holds that
$\leq_1 \circ \leq_2 \: = \: \leq_2 \circ \leq_1$.
\end{cor}

\begin{proof}
  Proposition~\ref{fileq} deals with most of these cases. The remaining ones
are straightforward: just note that $$\leq_t \circ
  \geq_t \: = \: \geq_t \circ \leq_t \: = \: B \times B \: = \: \leq_k \circ \geq_k \: = \: \geq_k \circ \leq_k.$$
\end{proof}

An easy consequence of the previous corollary is that for every $\leq_1, \leq_2
\ \in$ $\{ {\leq_t,} {\geq_t,} \leq_k, \geq_k \}$, the relation $\leq_1
\circ \leq_2$ is always transitive. This is so because we have 
%$$(\leq_1
%\circ \leq_2) \circ ( \leq_1 \circ \leq_2)  \: = \: \leq_1 \circ ( \leq_2
%\circ \leq_1) \circ \leq_2 \: = \: \leq_1 \circ ( \leq_1 \circ \leq_2) \circ
%\leq_2 \: = \: (\leq_1 \circ \leq_1) \circ ( \leq_2 \circ \leq_2) \: = \: \leq_1
%\circ \leq_2. $$ 
\begin{align*}
(\leq_1
\circ \leq_2) \circ ( \leq_1 \circ \leq_2)  \: & = \: {\leq_1} \circ ( \leq_2
\circ \leq_1) \circ {\leq_2} \\ & = \: {\leq_1} \circ ( \leq_1 \circ \leq_2) \circ
{\leq_2} \\ & = \: (\leq_1 \circ \leq_1) \circ ( \leq_2 \circ \leq_2) \\ & = \: \leq_1
\circ \leq_2.
\end{align*}
%\texttt{Fijate en como he arreglado los espacios antes y despues de $\circ$ \\ que no quedaban bien. }

Hence, $\leq_1 \circ \leq_2$ is a quasi-order (i.e., it
is a reflexive and transitive relation) compatible with all four lattice
operations. Compatibility  can be easily proved using  the interlacing
conditions, which  say that both $\leq_1$ and $\leq_2$ are
compatible with the four operations. This suggests that there may be an interest in studying the
equivalence relations determined by these quasi-orders.

%\texttt{No entiendo la frase del \'ultimo p\'arrafo que comienza con "This".  Consideras los elementos de la relacion de equivalencia 
%del preorden, \\ que no es la generada. La generada incluye al preorden, pues es la menor relacion de equivalencia que lo incluye. \\ La relacion de equivalencia del preorden
%es la formada por los pares 
%$\la a, b\ra$ tales que $\la a, b\ra$ y $\la b, a\ra$ pertenecen al preorden.\\
%De nuevo, es dif\'icil leer la proposici\'on}

%\texttt{Creo que seria mejor definir $\sim_1 = (\leq_t \circ \leq_k) \cap (\leq_t \circ \leq_k)^{-1}$ y analogmente $\sim_{2}$ primero (y eliminar la def. 1.5). $(\leq_t \circ \leq_k)^{-1}$ es la relaci\'on inversa de $(\leq_t \circ \leq_k)$. Esta definicion de relacion de equivalencia de un pre-orden es transparente y estandar. Despues formularia la proposicion asi:  $a \sim_1 b$ iff... Igualmente con $\sim_2$.    }

%\texttt{Umberto: He cambiado la frase que no se entendia y tambien la def. 1.4 segun tus sugerencias; tambien he intentado simplificar la prop. 1.5 para que quede visualmente mas clara.}

\begin{definition} \label{d:cong}
  Let $\Al[B] = \langle B, \leq_{t}, \leq_{k} \rangle$ be an
interlaced pre-bilattice and let $\leq^{-1}$ denote the inverse of the relation $\leq$. We denote by $\sim_1$ and $\sim_2$ the equivalence relations defined as follows: 
\begin{align*}
\sim_1 & \: = \: (\leq_t \circ \leq_k) \cap (\leq_t \circ \leq_k)^{-1} \\
\sim_2 & \: = \: (\geq_t \circ \leq_k) \cap (\geq_t \circ \leq_k)^{-1}.
\end{align*}
\end{definition} 

Obviously we have $a \sim_{1} b$ if and only if $\langle a,b \rangle, \langle b,a \rangle \in  {(\leq_t \circ \leq_k)}$, and similarly  $a \sim_{2} b$ means that $\langle a,b \rangle, \langle b,a \rangle \in  {(\geq_t \circ \leq_k)}$. Recalling the result of Corollary   \ref{cor:interlacingorders}, we see that in an interlaced pre-bilattice there are many equivalent ways of expressing these conditions. Some of them are contained in the following proposition:


\begin{proposition} \label{prop:symetrization}
Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus \rangle$ be an interlaced pre-bilattice. Then, for all $a, b \in B$: 

\begin{tabular}[c]{lllllllllllllllll}
\\
(i) && $a \sim_{1} b$      && $\Leftrightarrow$ && $a \lor b = a \otimes b$    && $\Leftrightarrow$ && $a \lor b \leq_t a \otimes b$ && $\Leftrightarrow$ \\
    &&   && $\Leftrightarrow$ && $a \oplus b = a \land b$    && $\Leftrightarrow$  && $a \oplus b \leq_k a \land b$. \\ \\
(ii) && $a \sim_{2} b$      && $\Leftrightarrow$ && $a \land b = a \otimes b$    && $\Leftrightarrow$ && $a \land b \geq_t a \otimes b$ && $\Leftrightarrow$ \\
    &&   && $\Leftrightarrow$ && $a \oplus b = a \lor b$    && $\Leftrightarrow$  && $a \oplus b \leq_k a \lor b$.  \\   
    \end{tabular} 
%\begin{enumerate}[(i)]
%  \item 
%    $\langle a,b \rangle, \langle b,a \rangle \in \: (\leq_t \circ \leq_k)$ \quad $\Leftrightarrow$ \quad
%    $a \lor b \leq_t a \otimes b$ \quad $\Leftrightarrow$ \quad
%    $a \lor b = a \otimes b$ \quad $\Leftrightarrow$ \quad\\
%    $\langle a,b \rangle, \langle b,a \rangle \in \: (\leq_k \circ \leq_t)$ \quad $\Leftrightarrow$ \quad
%    $a \oplus b \leq_k a \land b$ \quad $\Leftrightarrow$ \quad
%    $a \oplus b = a \land b$ \quad $\Leftrightarrow$ \quad\\
%    $\langle a,b \rangle, \langle b,a \rangle \in \: (\geq_t \circ \geq_k)$ \quad $\Leftrightarrow$ \quad
%    $a \land b \geq_t a \oplus b$ \quad $\Leftrightarrow$ \quad
%    $a \land b = a \oplus b$ \quad $\Leftrightarrow$ \quad\\
%    $\langle a,b \rangle, \langle b,a \rangle \in \: (\geq_k \circ \geq_t)$ \quad $\Leftrightarrow$ \quad
%    $a \otimes b \geq_k a \lor b$ \quad $\Leftrightarrow$ \quad
%    $a \otimes b = a \lor b$.

%  \item 
%    $\langle a,b \rangle, \langle b,a \rangle \in \: (\geq_t \circ \leq_k)$ \quad $\Leftrightarrow$ \quad
%    $a \land b \geq_t a \otimes b$ \quad $\Leftrightarrow$ \quad
%    $a \land b = a \otimes b$ \quad $\Leftrightarrow$ \quad\\
%    $\langle a,b \rangle, \langle b,a \rangle \in \: (\leq_k \circ \geq_t)$ \quad $\Leftrightarrow$ \quad
%    $a \oplus b \leq_k a \lor b$ \quad $\Leftrightarrow$ \quad
%    $a \oplus b = a \lor b$ \quad $\Leftrightarrow$ \quad\\
%    $\langle a,b \rangle, \langle b,a \rangle \in \: (\leq_t \circ \geq_k)$ \quad $\Leftrightarrow$ \quad
%    $a \lor b \leq_t a \oplus b$ \quad $\Leftrightarrow$ \quad
%    $a \lor b = a \oplus b$ \quad $\Leftrightarrow$ \quad\\
%    $\langle a,b \rangle, \langle b,a \rangle \in \: (\geq_k \circ \leq_t)$ \quad $\Leftrightarrow$ \quad
%    $a \otimes b \geq_k a \land b$ \quad $\Leftrightarrow$ \quad
%    $a \otimes b = a \land b$.
%\end{enumerate}
\end{proposition}

\begin{proof}
  By the Duality Principle and Proposition~\ref{fileq}, it is sufficient to prove the first line of (i), i.e. that
   $\langle a,b \rangle, \langle b,a \rangle \in \: \leq_t \circ \leq_k$
  iff $a \lor b \leq_t a \otimes b$ iff $a \lor b = a \otimes b$. And
  this is an easy consequence of Proposition~\ref{fileq} together
  with the fact that, by the interlacing
  conditions, $a \otimes b \leq_t a \lor b$.
\end{proof}

Hence, two elements of an interlaced pre-bilattice are related by $\sim_{1}$ whenever any of the conditions in the first
  statement of Proposition~\ref{prop:symetrization} holds; similarly,
  the equivalence relation $\sim_2$ can be defined by the conditions
  of the second statement. 

The following proposition contains the main results of this section: a direct decomposition of interlaced pre-bilattices, a representation as pre-bilattice products of two lattices and a characterization of the congruences. In the proof we shall use the fact that all varieties of (pre-)bilattices are congruence-distributive: this is immediate, since lattices are congruence-distributive (see \cite[p.~87]{BuSa00}) and this property is preserved by expansions of the language.


\begin{proposition} \label{prop:interlaced_pbl}
Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus \rangle$ be an
interlaced pre-bilattice. Then, 
\begin{enumerate}[(i)]
  \item $\sim_1$ and $\sim_2$ are congruences of $\Al[B]$.
  \item $\Al[B]/\!\!\sim_1$ and $\Al[B]/\!\!\sim_2$ are interlaced
    pre-bilattices.
  \item In $\Al[B]/\!\!\sim_1$, %it holds that
    the knowledge order coincides with the truth order. 
    %That is, $\langle B, \otimes, \oplus \rangle /\!\!\sim_1 =  \langle B, \land, \lor \rangle /\!\!\sim_1$.
  \item In $\Al[B]/\!\!\sim_2$, %it holds that 
    the knowledge order is the dual of the truth order. % That is, $\langle B, \otimes, \oplus \rangle /\!\!\sim_2 =  \langle B, \lor, \land \rangle /\!\!\sim_2$.
  \item $\sim_1$ and $\sim_2$ is a pair of factor congruences of
    $\Al[B]$ \\ (i.e., $\sim_1 \cap \sim_2$ is the identity relation and
    $\sim_1 \circ \sim_2$ is the total relation $\nabla$).
  \item $\Al[B]$ is isomorphic to the direct product $\Al[B]/\!\!\sim_1
    \times \: \Al[B]/\!\!\sim_2$.
  \item $\Al[B]$ is isomorphic to the product pre-bilattice $(\langle B,
    \otimes, \oplus \rangle /\!\!\sim_1) \odot  (\langle B, \otimes,
    \oplus \rangle /\!\!\sim_2)$.
  \item $\langle \Con(\Al[B]) , \subseteq \rangle \: \cong \: \langle \Con (\langle B, \otimes, \oplus \rangle / \!\!\sim_1), \subseteq \ra
    \times \la \Con (\langle B, \otimes, \oplus \rangle / \!\!\sim_2),
    \subseteq \rangle$.
  \item $\langle \Con(\Al[B]) , \subseteq \rangle$ is isomorphic to 
    $\langle [\sim_1, \nabla]_{\Con(\Al[B])}, \subseteq \ra \times \la [\sim_2,
    \nabla]_{\Con(\Al[B])}, \subseteq \rangle$, where \\ $[\sim_i,
    \nabla]_{\Con(\Al[B])} = \{ \theta \in \Con (\Al[B]): \: \sim_i \:
    \subseteq \theta \}$.
  \item $\Con(\Al[B]) = \Con (\langle B, \land, \lor \rangle) = \Con (\langle B, \otimes, \oplus \rangle)$.
    

\end{enumerate}
\end{proposition}

%\texttt{Eliminaria en (3) y (4) la frase explicativa que empieza con "That is"}

\begin{proof}
  (i). This is obvious from the fact that each one of these two relations
  is the equivalence relation of a quasi-order compatible with the operations.

  (ii). Immediate, since $\IPBL$ is a variety.

  (iii). It is enough to note that $a \land b \sim_1 a \otimes b$ (or
  that $a \lor b \sim_1 a \oplus b$). By the interlacing conditions we
  know that $a \land b \leq_t a \otimes b \leq_k a \land b$. Hence,
  $\langle  a \land b , a \otimes b \rangle \in \: 
  \leq_t \circ \leq_k$ and $\langle a \otimes b , a \land b \rangle \in
  \: \leq_t \circ \leq_k$. Thus, it holds that $a \land
  b \sim_1 a \otimes b$.

  (iv). It suffices to check that $a \land b \sim_2 a \oplus b$ (or
  that $a \lor b \sim_2 a \otimes b$). By the interlacing conditions we
  know that $a \land b \leq_t a \oplus b \leq_k a \land b$. Hence,
  $\langle  a \land b , a \oplus b \rangle \in \: 
  \leq_t \circ \leq_k$ and $\langle a \oplus b , a \land b \rangle \in
  \: \leq_t \circ \leq_k$. Thus, it holds that $a \land
  b \sim_2 a \oplus b$.

  (v). Let us  first consider the case of the intersection.
  Let us assume that $a \sim_1 b$ and $a \sim_2 b$. Then, by
  Proposition~\ref{prop:symetrization} we know that $a \lor b = a
  \otimes b$ and $a \land b = a \otimes b$. Therefore, $a \lor b = a
  \land b$. Hence $a = b$. In order to prove that $\sim_1 \circ
  \sim_2$ is the total relation, it is enough to
  check that the element $c = (a \land (a \oplus b)) \otimes (b \lor (a
  \oplus b))$ satisfies that $a \sim_1 c$ and $b \sim_2 c$. Using
  previous items in this proposition it is easy to see that 
  $$
  c = (a \land (a \oplus b)) \otimes (b \lor (a
  \oplus b)) \sim_1 (a \land (a \lor b)) \land (b \lor (a
  \lor b)) \sim_1 a \land (a \lor b) \sim_1 a
  $$
  and that
  $$
  c = (a \land (a \oplus b)) \otimes (b \lor (a
  \oplus b)) \sim_2 (a \land (a \land b)) \lor (b \lor (a
  \land b)) \sim_2 (a \land b) \lor b \sim_2 b.
  $$

  (vi). By (v) and \cite[Theorem~II.7.5]{BuSa00}.

  (vii). As observed in Chapter \ref{ch:intro}, %1
 for any two lattices $\Al[L_1]$ and $\Al[L_2]$, the product  pre-bilattice $\Al[L_1] \odot \Al[L_2]$ coincides with the direct product
$\Al[L_1^{++}] \times \Al[L_2^{-+}]$. The result then follows from the fact that $\Al[B]/\!\!\sim_1 = (\langle B, \otimes, \oplus \rangle /\!\!\sim_1)^{++}$ and $\Al[B]/\!\!\sim_2 = {(\langle B, \otimes, \oplus \rangle /\!\!\sim_1)^{+-}}$.
  
  %This holds because $\Al[B]/\!\!\sim_1 \times \: \Al[B]/\!\!\sim_2$ is exactly $$(\langle B, \otimes, \oplus \rangle /\!\!\sim_1) \odot (\langle B, \otimes, \oplus \rangle /\!\!\sim_2).$$ 
  
  Notice also that 
  $$(\langle B, \otimes, \oplus \rangle /\!\!\sim_1) \cong (\langle B,
  \land, \lor \rangle /\!\!\sim_1)$$ and $$(\langle B, \otimes,
  \oplus \rangle /\!\!\sim_2) \cong (\langle B, \lor, \land \rangle
  /\!\!\sim_2).$$
    
  (viii). As we have observed, pre-bilattices are congruence-distributive; hence they also enjoy the Fraser-Horn-Hu property (see \cite[Corollary~1]{FrHo70}). This means that the lattice of congruences of a direct product is isomorphic to the direct
  product of the lattices of congruences of the factor algebras. We have then that $$\Con(\Al[B]) \cong \Con ( \Al[B]/\!\!\sim_1 \times \:
  \Al[B]/\!\!\sim_2 ) \cong \Con( \Al[B]/\!\!\sim_1) \times \: \Con(
  \Al[B]/\!\!\sim_2 ).$$ 
  To finish the proof it is enough to observe that,
  as a consequence of (iii)  and (iv), it holds that if $i \in \{ 1, 2 \}$ then $\Con(
  \Al[B]/\!\!\sim_i ) = \Con (\langle B, \otimes, \oplus \rangle /
  \!\!\sim_i )$.

  (ix). The beginning of this proof is the same one than for the previous
  item.  In order to finish it we use that, by
  \cite[Theorem~II.6.20]{BuSa00}, if $i \in \{ 1, 2 \}$ then $\Con(
  \Al[B]/\!\!\sim_i) \cong [\sim_i, \nabla]$.

%  (x). By the Duality Principle it suffices to prove that $\Con(\Al[B]) =
%  \Con (\langle B, \otimes, \oplus \rangle)$. Recall that, as observed in (viii), if $i \in \{ 1, 2 \}$ then ${\Con(
%  \Al[B]/\!\!\sim_i )} = {\Con (\langle B, \otimes, \oplus \rangle /
%  \!\!\sim_i )}$. Using the Fraser-Horn-Hu property, we have 
%  \begin{align*} 
% \Con(\Al[B]) & \cong \Con ( \Al[B]/\!\!\sim_1 \times \: \Al[B]/\!\!\sim_2 )  \\
%    &  \cong \Con( \Al[B]/\!\!\sim_1) \times \: \Con(\Al[B]/\!\!\sim_2 ) \\
%    & \cong \Con (\langle B, \otimes, \oplus \rangle / \!\!\sim_1 ) \times \Con (\langle B, \otimes, \oplus \rangle / \!\!\sim_2 ) \\
%    & \cong \Con (\langle B, \otimes, \oplus \rangle). 
%\end{align*}
 
  (x). Clearly, it is enough to prove that $\Con (\langle B, \land, \lor \rangle) = \Con (\langle B, \otimes, \oplus \rangle)$. We will show that $ \Con (\langle B, \otimes, \oplus \rangle) \subseteq \Con (\langle B, \land, \lor \rangle)$, so the result will follow by duality.  Using (vii), we may identify $\Al[B]$ with its isomorphic image  ${(\langle B,
    \otimes, \oplus \rangle /\!\!\sim_1)} \odot  {(\langle B, \otimes,
    \oplus \rangle /\!\!\sim_2)}$. Let us use the following notation: $\langle B, \otimes, \oplus \rangle /\!\!\sim_1 \: = \la B_{1}, \otimes_{1}, \oplus_{1}\ra $ and $\langle B, \otimes, \oplus \rangle /\!\!\sim_2 \: = \la B_{2}, \otimes_{2}, \oplus_{2}\ra $.
    
 Assume $\theta \in \Con (\langle B, \otimes, \oplus \rangle)$ and $\la \la a_1, a_{2} \ra, \la b_1, b_{2} \ra \ra \in \theta $ for some $a_{1}, b_{1} \in B_{1}$ and $a_{2}, b_{2} \in B_{2}$. It is easy to check that, for any   $\la c_{1}, c_{2} \ra \in B$, it holds that $\la a_1, a_{2} \ra \land \la c_{1}, c_{2} \ra = (\la a_1, a_{2} \ra \otimes d) \oplus e$ and $\la b_1, b_{2} \ra \land \la c_{1}, c_{2} \ra = (\la b_1, b_{2} \ra \otimes d) \oplus e$, where $d = \la c_{1}, a_{2} \oplus_{2} b_{2} \ra $ and  $e = \la a_{1} \otimes_{1} b_{1} \otimes_{1} c_{1}, c_{2} \ra $. Since we are in a lattice, this implies that $\theta$ is compatible with $\land$. The case of $\lor$ can be proved in the same way, taking $d = \la a_{1} \oplus_{1} b_{1}, c_{2} \ra $ and  $e = \la c_{1}, a_{2} \otimes_{2} b_{2} \otimes_{2} c_{2} \ra $. Hence, we conclude that $\theta \in \Con (\langle B, \land, \lor \rangle)$.
%
\end{proof} 

%We may observe that the last item of Proposition \ref{prop:interlaced_pbl} could be strengthened, for the isomorphism involved is indeed the identity, so that we have  $\Con(\Al[B]) = \Con (\langle B, \land, \lor \rangle) = \Con
%    (\langle B, \otimes, \oplus \rangle)$. 
%    
    As a corollary of Proposition \ref{prop:interlaced_pbl}  (vii), we obtain the generalized version of the Representation Theorem: 

\begin{thm}[Representation, 1]
  \label{thm:representation}
  Let $\Al[B]$ be a pre-bilattice. The following statements are
  equivalent.
  \begin{enumerate}[(i)]
    \item $\Al[B]$ is an interlaced pre-bilattice.
    \item There are two lattices $\Al[L_1]$ and $\Al[L_2]$ such that
      $\Al[B]$ is isomorphic to $\Al[L_1] \odot \Al[L_2]$.
  \end{enumerate}
\end{thm}

An interesting consequence of Proposition \ref{prop:interlaced_pbl} (x) is that any
property that only depends on the lattice of congruences transfers
straightforwardly from interlaced pre-bilattices to lattices and viceversa (this can be regarded as a generalization of the results of \cite{MoPiSlVo00} mentioned in Chapter %1
\ref{ch:intro}). 

% \texttt{No seria mejor decir : an interlaced pre-bilattice $\Al[B]$ is subdirectly \\ irreducible iff some (in fact both) of its lattice reducts\\  (the truth or the knowledge one)  is subdirectly irreducible.}

For instance, an
interlaced pre-bilattice $\Al[B] = \langle B, \land, \lor, \otimes, \oplus \rangle$ is subdirectly irreducible  if and only if some (hence both) its lattice reducts  $ \langle B, \land, \lor \rangle$ and $ \langle B, \otimes, \oplus \rangle$  are subdirectly irreducible lattices; it is directly indecomposable as a pre-bilattice if and only if its lattice reducts are, and so on.
Note also that, using the Fraser-Horn-Hu
property~\cite{FrHo70} as in this Proposition \ref{prop:interlaced_pbl} (x), we get as a
consequence that $\Con (\Al[L_1] \odot \Al[L_2]) \cong \Con(\Al[L_1])
\times \Con(\Al[L_2])$.

\begin{rem}   \label{rem:sublat}
Comparing Theorem \ref{thm:representation} with its analogue for bounded pre-bilattices (Theorem \ref{thm:reprpre}), one sees that in the bounded case  the decomposition is achieved by constructing two lattices that are in fact sub-pre-bilattices of the original (pre-)bilattice. This nice feature is  apparently lost when we come to the unbounded case. However, using Theorem \ref{thm:representation}, it is not difficult to see that one could prove the following.
%
Let $\Al[B] = \Al[L_1] \odot \Al[L_2]$ be an interlaced pre-bilattice and let us fix some $a  \in B $. Let 
$[a]_{1} = \{ b  \in B : a \sim_{1} b \}$ and $[a]_{2} = \{ b  \in B : a \sim_{2} b \}$. If we let $a = \la a_{1}, a_{2} \ra $, then we have that:
\begin{enumerate}[(i)]
  \item $[a]_{1} = \{ \la a_{1}, b_{2} \ra : b_{2} \in L_{2} \}$ and $[a]_{2} = \{ \la b_{1}, a_{2} \ra : b_{1} \in L_{1} \}$ 
  \item $[a]_{1}$ and $[a]_{2}$ are universes of sub-pre-bilattices of $\Al[B]$ 
  \item $ \la [a]_{1}, \otimes, \oplus \ra = \la [a]_{1}, \lor, \land \ra$ and $ \la [a]_{2}, \otimes, \oplus \ra = \la [a]_{2}, \land, \lor \ra$
    \item $ \Al[L_1]  \cong \la [a]_{2}, \otimes, \oplus \ra$ and $ \Al[L_2]  \cong \la [a]_{1}, \otimes, \oplus \ra $. 
%
\end{enumerate}
The isomorphisms $f_{1} : L_{1} \longrightarrow [a]_{2} $ and $f_{2} : L_{2} \longrightarrow [a]_{1} $ are defined in the obvious way: $f_{1} (b_{1}) = \la b_{1}, a_{2} \ra$ for all $b_{1} \in L_{1}$ and $f_{2} (b_{2}) = \la a_{1}, b_{2} \ra$ for all $b_{2} \in L_{2}$. 



%$[\la a_{1}, a_{2} \ra]_{1} = \{ \la b_{1}, b_{2} \ra \in L_{1} \times L_{2} : \la a_{1}, a_{2} \ra \sim_{1} \la b_{1}, b_{2} \ra \}$ and 

%For our purposes, it is interesting to note that in both cases the decomposition is achieved by constructing two lattices that are in fact sub-pre-bilattices of the original (pre-)bilattice: this nice feature shall be lost when we come to representation of unbounded pre-bilattices, but we will be able to regain it in the case of unbounded bilattices.
 
\end{rem}

The following theorem provides another generalization of some known results on bounded interlaced pre-bilattices.

%\texttt{He a\~nadido esta frase: }

Let $\varepsilon(\sqcap,\sqcup)$ be an equation in the language of lattices. Then if $\{ \circ, \bullet \}$ are connectives of the language of pre-bilattices, $\varepsilon(\circ, \bullet)$ is the result of substituting $\circ$ and $\bullet$ respectively for $\sqcap$ and $\sqcup$.  

\begin{thm}
  \label{thm:representation_eq}
  Let  $\Al[B] = \langle B, \land, \lor, \otimes, \oplus \rangle$  be a pre-bilattice and let $\varepsilon(\sqcap,\sqcup)$ be an
  equation in the language of lattices. The following statements are
  equivalent:
  \begin{enumerate}
    \item $\Al[B]$ is interlaced and $\Al[B]
      \models \{ \varepsilon(\land,\lor), \varepsilon(\lor,\land)
      ,\varepsilon(\otimes,\oplus),  \varepsilon(\oplus,\otimes) \}$.
    \item $\Al[B]$ is interlaced and $\Al[B]
      \models \{ \varepsilon(\land,\lor), \varepsilon(\lor,\land) \}$.
    \item $\Al[B]$ is interlaced and $\Al[B]
      \models \{ \varepsilon(\otimes,\oplus), \varepsilon(\oplus,\otimes) \}$.
    \item There are two lattices $\Al[L_1]$ and $\Al[L_2]$ such that
      $\Al[L_1] \models \{ \varepsilon(\sqcap,\sqcup),
      \varepsilon(\sqcup, \sqcap) \}$, $\Al[L_2] \models \{
      \varepsilon(\sqcap,\sqcup), \varepsilon(\sqcup, \sqcap) \}$ and
      $\Al[B]$ is isomorphic to $\Al[L_1] \odot \Al[L_2]$.
  \end{enumerate}
\end{thm}

\begin{proof}
  By duality, we can  skip the second condition and just check that all the remaining ones are equivalent:

  $1 \Rightarrow 3:$ This is trivial.

  $3 \Rightarrow 4:$ By 
  Proposition \ref{prop:interlaced_pbl} (vii).

  $4 \Rightarrow 1:$ This follows from the fact that $\Al[L_1] \odot
  \Al[L_2] \cong \Al[L_1^{++}] \times \Al[L_2^{-+}]$.
\end{proof}

A consequence of Theorem \ref{thm:representation_eq} is a result which is well-known for bounded pre-bilattices: 

\begin{proposition} \label{prop:distributive_bl}
An interlaced pre-bilattice is distributive if and only if its t-lattice (or, equivalently, its k-lattice) reduct is distributive.
\end{proposition} 

For the case of distributive pre-bilattices, it is easy to see that from Theorem  \ref{thm:representation} we may obtain another representation result:

\begin{proposition} \label{p:rep_dist}
Every distributive pre-bilattice is isomorphic to a pre-\-bi\-lattice of sets.
\end{proposition} 

\begin{proof}
By Theorem  \ref{thm:representation}, any distributive pre-bilattice $\Al[B] $ is isomorphic to $\Al[L_1] \odot
  \Al[L_2]$, where $\Al[L_1]$ and $\Al[L_1]$ are distributive lattices. It is a well-known result of lattice theory that any distributive lattice is isomorphic to a lattice of sets (see \cite[Theorem~II.1.19]{Gr78}). Hence we have $\Al[L_1] \cong \Al[L_1']$ and $\Al[L_2] \cong \Al[L_2']$, where $\Al[L_1']$ and  $\Al[L_2']$ are lattices of sets. So $\Al[L_1'] \odot
  \Al[L_2']$ is a pre-bilattice of sets and $\Al[B] \cong \Al[L_1'] \odot
  \Al[L_2']$.
\end{proof}

In Section \ref{sec:dis} we will see that the previous result can also be obtained directly by considering the ``bifilters'' of a pre-bilattice (i.e.\ subsets that are lattice filters of both orders).

%\texttt{Quiza vale la pena poner lo anterior como una proposici\'on.}

\section{Representation Theorem for bilattices}
\label{sec:repbil}


In this section we deal with the Representation Theorem
for the case of interlaced bilattices. The main difference from the previous section is, of course, that the language has been expanded with a
negation operation carrying some additional properties. We will see that
the main consequence of this expansion is that the two factor lattices of the  product bilattice obtained turn out to be isomorphic. This result also was well-known for the case of bounded interlaced bilattices.

First of all, let us point out that negation affects the Duality Principle.
In fact, in the presence of negation, duality only allows to replace $\leq_t$ with
$\geq_t$, and to replace $\leq_k$ with $\geq_k$. It is no more allowed to
change $\leq_t$ with $\leq_k$, because negation has to be antimonotonic with
respect to $\leq_t$ but monotonic with respect to $\leq_k$.

The proof of the Representation Theorem for bilattices is essentially the same 
as that described in the previous section: that is, it uses
the congruences $\sim_1$ and $\sim_2$ of the pre-bilattice reduct. Note, however, that
 it is not true that $\sim_1$ and $\sim_2$ are compatible
with the negation operator, so the quotients obtained will not be algebras of the same type.

The following lemma clarifies the behaviour of the negation with respect to the two congruences and will allow to prove our main claim:

\begin{lem}
  \label{lem:cong_bl}
  Let $\Al[B]$ be an interlaced bilattice. Then, for every $a, b \in B$
  it holds that
  \begin{enumerate}[(i)]
    \item $\quad a \sim_1 b\:$ iff $\: \neg a \sim_2 \neg b$.
    \item $\quad  a \sim_2 b\: $ iff $\: \neg a \sim_1 \neg b$.
  \end{enumerate}
\end{lem} 

\begin{proof}
  This follows from Proposition~\ref{prop:symetrization} together with
  De Morgan laws.
\end{proof}


%\texttt{Yo pondria los isomorfismos en el enunciado. Por ejemplo:  The map $f: B/{\sim_1} \to B/{\sim_2}$ given by
%$$f([a]_{\sim_1}) = [\neg a]_{\sim_2}$$ is an isomorphism between $\langle B, \otimes, \oplus \rangle /\!\!\sim_1$ and $ \langle B,\otimes, \oplus \rangle /\!\!\sim_2$.  Es mas informativo. \\ Al quedar los enunciados mas largos, pudes dividir la proposicion en dos. Una con (1) y (2) y la otra con los items sobre los reticulos de congruencias. }

%\texttt{Umberto: He dividido la proposicion segun tus sugerencias y he puesto los isomorfismos en el enunciado. El unico que he dejado en la prueba es el de la Prop. \ref{prop:interbl_cong} (i), porque me parecia demasiado largo explicar en el enunciado que todo interlaced bilattice se puede ver como una potencia de un mismo reticulo etc.}


We are now able to state our main claim:

\begin{thm} [Representation, 2]
\label{thm:interlaced_bl}
Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus, \neg \rangle$ be an
interlaced bilattice and $a \in B$. Then:

\begin{enumerate}[(i)]
  \item $\langle B, \otimes, \oplus \rangle /\!\!\sim_1$ and $ \langle B,
    \otimes, \oplus \rangle /\!\!\sim_2$ are isomorphic through the map $f: B/{\sim_1} \longrightarrow B/{\sim_2}$ defined as
$$f([a]_{\sim_1}) = [\neg a]_{\sim_2}.$$
  \item $\Al[B]$ is isomorphic to the product bilattice $(\langle B,
    \otimes, \oplus \rangle /\!\!\sim_1) \odot  (\langle B, \otimes,
    \oplus \rangle /\!\!\sim_1)$ through the map $h: B \longrightarrow B/{\sim_1} \times B/{\sim_1} $ defined as
$$h(a) = \la [a]_{\sim_1}, [\neg a]_{\sim_1} \ra.$$

  \end{enumerate}
\end{thm}

\begin{proof}
  (i). By Lemma~\ref{lem:cong_bl} it is clear that the map $f$, defined by the
  assignment $$[a]_{\sim_1} \longmapsto [\neg a]_{\sim_2}$$ is an
  isomorphism.
  
  (ii). By Proposition~\ref{prop:interlaced_pbl} (vii), we know that the map
  $a \longmapsto \langle [a]_{\sim_1}, [a]_{\sim_2} \rangle$ is an
  isomorphism between $\langle B, \land, \lor, \otimes, \oplus \rangle$
  and $(\langle B, \otimes, \oplus \rangle /\!\!\sim_1) \odot  (\langle
  B, \otimes, \oplus \rangle /\!\!\sim_2)$, where this last product is taken
  as a pre-bilattice. Therefore, by the previous item it follows that the
  map $a \longmapsto \langle [a]_{\sim_1}, [\neg a]_{\sim_1} \rangle$ is
  an isomorphism between $\langle B, \land, \lor, \otimes, \oplus
  \rangle$ and $(\langle B, \otimes, \oplus \rangle /\!\!\sim_1) \odot
  (\langle B, \otimes, \oplus \rangle /\!\!\sim_1)$. Thus, it suffices
  to prove that this last map is also a homomorphism of the negation
  operator, which is trivial.
\end{proof}

With respect to the lattice of congruences of interlaced bilattices, we may state the following results.

\begin{proposition} \label{p:interbl_cong}
Let $ \Al[L] \odot \Al[L]$ be a product bilattice. Then   $\Con (\Al[L] \odot \Al[L]) \cong \Con (\Al[L])$.
\end{proposition} 

\begin{proof}
Let $\Al[L] = \langle L, \sqcap, \sqcup \rangle$. By Proposition~\ref{prop:interlaced_pbl} (viii), in the  case  of the product pre-bilattice we have  $\Con
  (\langle L, \sqcap, \sqcup \rangle \odot \langle L, \sqcap, \sqcup
  \rangle) \cong \Con (\langle L, \sqcap, \sqcup \rangle) \times
  \Con(\langle L, \sqcap, \sqcup \rangle)$ under the assignment $\theta
  \longmapsto \langle \pi_1 (\theta), \pi_2 (\theta) \rangle$, where
  $\pi_i$ refers to $i$th-projection. If $\theta \in \Con
  (\langle L, \sqcap, \sqcup \rangle \odot \langle L, \sqcap, \sqcup
  \rangle)$ is also a congruence with respect to the negation operator,
  then $\pi_1[\theta] = \pi_2 [\theta]$ because 
  \begin{center}
    $\langle a_1, a_2 \rangle \in \pi_1[\theta]$ \quad iff \quad 
    there is some $b \in L$ such that $\langle a_1, b \rangle \theta
    \langle a_2, b \rangle$ \quad iff \quad\\
    there is some $b \in L$ such that $\langle b,a_1 \rangle \theta
    \langle b,a_2 \rangle$ \quad iff \quad
    $\langle a_1, a_2 \rangle \in \pi_2[\theta]$.
  \end{center} 
  Hence, it is clear that the map $\theta \longmapsto
  \pi_1[\theta]$ is an isomorphism between the lattices $\Con (\langle L, \sqcap, \sqcup
  \rangle \odot \langle L, \sqcap, \sqcup \rangle)$ and $\Con (\langle
  L, \sqcap, \sqcup \rangle)$.
\end{proof}

\begin{proposition} \label{prop:interbl_cong}
Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus, \neg \rangle$ be an
interlaced bilattice. Then: 
\begin{enumerate}[(i)]
    \item $\Con(\Al[B]) \cong \Con (\langle B, \otimes, \oplus \rangle / \!\!\sim_1)$.
    
  \item $\Con(\Al[B]) = \Con (\langle B, \land, \lor, \neg \rangle) = \Con
    (\langle B, \otimes, \oplus, \neg \rangle)$.
     
     \item $\Con(\Al[B]) = \Con (\langle B, \land, \neg \rangle) = \Con
    (\langle B, \lor,  \neg \rangle)$.
\end{enumerate}
\end{proposition}

\begin{proof}
  (i).  By Theorem \ref{thm:interlaced_bl} (ii), we know that $$\Al[B] \cong {\langle B, \otimes, \oplus \rangle / \!\!\sim_1} \odot {\langle B, \otimes, \oplus \rangle / \!\!\sim_1}.$$ Hence the result follows from Proposition \ref{p:interbl_cong}.
  
%   it is enough to prove that $\Con (\Al[L] \odot
%  \Al[L]) \cong \Con (\Al[L])$, where $\Al[L] = \langle L,
%  \sqcap, \sqcup \rangle$ is a lattice. By Proposition~\ref{prop:interlaced_pbl} (viii), we know that in the pre-bilattice case  $\Con
%  (\langle L, \sqcap, \sqcup \rangle \odot \langle L, \sqcap, \sqcup
%  \rangle) \cong \Con (\langle L, \sqcap, \sqcup \rangle) \times
%  \Con(\langle L, \sqcap, \sqcup \rangle)$ under the assignment $\theta
%  \longmapsto \langle \pi_1 (\theta), \pi_2 (\theta) \rangle$, where
%  $\pi_i$ refers to $i$th-projection. If $\theta \in \Con
%  (\langle L, \sqcap, \sqcup \rangle \odot \langle L, \sqcap, \sqcup
%  \rangle)$ is also a congruence with respect to the negation operator,
%  then $\pi_1[\theta] = \pi_2 [\theta]$ because 
%  \begin{center}
%    $\langle a_1, a_2 \rangle \in \pi_1[\theta]$ \quad iff \quad 
%    there is some $b \in L$ such that $\langle a_1, b \rangle \theta
%    \langle a_2, b \rangle$ \quad iff \quad\\
%    there is some $b \in L$ such that $\langle b,a_1 \rangle \theta
%    \langle b,a_2 \rangle$ \quad iff \quad
%    $\langle a_1, a_2 \rangle \in \pi_2[\theta]$.
%  \end{center} 
%  Therefore, it is obvious that the map $\theta \longmapsto
%  \pi_1[\theta]$ is an isomorphism between the lattices $\Con (\langle L, \sqcap, \sqcup
%  \rangle \odot \langle L, \sqcap, \sqcup \rangle)$ and $\Con (\langle
%  L, \sqcap, \sqcup \rangle)$.

  (ii). This is an easy consequence
  Proposition~\ref{prop:interlaced_pbl} (x).
  
  (iii). Follows easily from (ii), using De Morgan's laws.
%%
\end{proof}
%
%As for Proposition~\ref{prop:interlaced_pbl} (x), let us note that the previous result could be strengthened, in the sense that we have 
%$$\Con(\Al[B]) = \Con (\langle B, \land, \lor, \neg \rangle) = \Con
%    (\langle B, \otimes, \oplus, \neg \rangle) = \Con (\langle B, \land, \neg \rangle). $$



%\begin{proposition} \label{prop:interlaced_bl}
%Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus, \neg \rangle$ be an
%interlaced bilattice. Then, 
%\begin{enumerate}
%  \item $\langle B, \otimes, \oplus \rangle /\!\!\sim_1 \: \cong \: \langle B,
%    \otimes, \oplus \rangle /\!\!\sim_2$.
%  \item $\Al[B]$ is isomorphic to the product bilattice $(\langle B,
%    \otimes, \oplus \rangle /\!\!\sim_1) \odot  (\langle B, \otimes,
%    \oplus \rangle /\!\!\sim_1)$.
%  \item $\Con(\Al[B]) \cong \Con (\langle B, \otimes, \oplus \rangle / \!\!\sim_1)$.
%    
%  \item $\Con(\Al[B]) = \Con (\langle B, \land, \lor, \neg \rangle) = \Con
%    (\langle B, \otimes, \oplus, \neg \rangle)$.
%     \item $\Con(\Al[B]) = \Con (\langle B, \land, \neg \rangle) = \Con
%    (\langle B, \lor,  \neg \rangle)$.

%\end{enumerate}
%\end{proposition}


%\begin{proof}
%  1. By Lemma~\ref{lem:cong_bl} it is clear that the map defined by the
%  assignment $[a]_{\sim_1} \longmapsto [\neg a]_{\sim_2}$ is an
%  isomorphism.
%  
%  2. Due to Proposition~\ref{prop:interlaced_pbl} we know that the map
%  $a \longmapsto \langle [a]_{\sim_1}, [a]_{\sim_2} \rangle$ is an
%  isomorphism between $\langle B, \land, \lor, \otimes, \oplus \rangle$
%  and $(\langle B, \otimes, \oplus \rangle /\!\!\sim_1) \odot  (\langle
%  B, \otimes, \oplus \rangle /\!\!\sim_2)$ (this last product is taken
%  as a pre-bilattice). Therefore, by the previous item we know that the
%  map $a \longmapsto \langle [a]_{\sim_1}, [\neg a]_{\sim_1} \rangle$ is
%  an isomorphism between $\langle B, \land, \lor, \otimes, \oplus
%  \rangle$ and $(\langle B, \otimes, \oplus \rangle /\!\!\sim_1) \odot
%  (\langle B, \otimes, \oplus \rangle /\!\!\sim_1)$. Thus, it suffices
%  to prove that this last map is also a homomorphism of the negation
%  operator; and this is trivial.

%  3. By the previous item it is enough to prove that $\Con (\Al[L] \odot
%  \Al[L]) \cong \Con (\Al[L])$. Let $\Al[L]$ be the lattice $\langle L,
%  \sqcap, \sqcup \rangle$. We know from the pre-bilattice case (see a
%  paragraph below Proposition~\ref{prop:interlaced_pbl}) that $\Con
%  (\langle L, \sqcap, \sqcup \rangle \odot \langle L, \sqcap, \sqcup
%  \rangle) \cong \Con (\langle L, \sqcap, \sqcup \rangle) \times
%  \Con(\langle L, \sqcap, \sqcup \rangle)$ under the assignment $\theta
%  \longmapsto \langle \pi_1 (\theta), \pi_2 (\theta) \rangle$.  Here
%  $\pi_i$ refers to $i$th-projection. If $\theta \in \Con
%  (\langle L, \sqcap, \sqcup \rangle \odot \langle L, \sqcap, \sqcup
%  \rangle)$ is also a congruence with respect to the negation operator
%  then $\pi_1[\theta] = \pi_2 [\theta]$ because 
%  \begin{center}
%    $\langle a_1, a_2 \rangle \in \pi_1[\theta]$ \quad iff \quad 
%    there is some $b \in L$ such that $\langle a_1, b \rangle \theta
%    \langle a_2, b \rangle$ \quad iff \quad\\
%    there is some $b \in L$ such that $\langle b,a_1 \rangle \theta
%    \langle b,a_2 \rangle$ \quad iff \quad
%    $\langle a_1, a_2 \rangle \in \pi_2[\theta]$.
%  \end{center} 
%  Therefore, it is obvious that the map $\theta \longmapsto
%  \pi_1[\theta]$ is an isomorphism between the lattices $\Con (\langle L, \sqcap, \sqcup
%  \rangle \odot \langle L, \sqcap, \sqcup \rangle)$ and $\Con (\langle
%  L, \sqcap, \sqcup \rangle)$.

%  4. This is an easy consequence
%  Proposition~\ref{prop:interlaced_pbl} (10).
%  
%  5. Follows easily from (4), using De Morgan's laws.
%\end{proof}

Thanks to the presence of negation,  it is possible to give an
  alternative and straightforward proof of the Representation Theorem for interlaced bilattices. Like the preceding one, this proof does not use the boundedness assumption, and it also has the advantage that, as in the bounded case, the lattice factor we obtain is a sublattice of the original bilattice. Loosely speaking, the idea of the proof is also based on a projection of sorts: but in this case we are projecting each element of the bilattice on the ``vertical'' axis (the one that joins $\bot$ to $\top$ in the Hasse diagrams depicting bilattices).
 
  
  
  Given a bilattice $\Al[B]$, we consider the set $$\Reg(\Al[B]) = \{ a \in B: a = \neg a\}$$ of \emph{regular} elements,
  defined as those that are fixed points of the negation operator. Using De Morgan's laws, it is easy to check that this set is closed under $\otimes,
  \oplus$ and $\neg$, hence  is a sublattice of the k-lattice of $\Al[B]$. 
  %Thus, it makes sense to consider the lattice $\Reg(\Al[B]) = \la \Reg(B), \otimes, \oplus \ra$ 
  Now, to every $a \in B$ we associate a regular element according to the following definition: $$\reg(a) = (a \lor
  (a \otimes \neg a)) \oplus \neg (a \lor (a \otimes \neg a)).$$ 
  
  Clearly $\reg(a)$ is always a regular element. The following properties are also easily proved:
  
  %\texttt{Yo lo pondria como Lemma o como Proposition}
  
  \begin{proposition} \label{prop:regular}
  Let $\Al[B]= \la B, \land, \lor, \otimes, \oplus, \neg \ra$ be an interlaced bilattice. Then, for all $a, b \in B$:
\begin{enumerate}[(i)]
    \item $a \in \Reg(\Al[B])$ \: iff \: $a = \reg(a)$ \: iff \: $a =
      \reg(b)$ for some $b \in B$,
    \item $a \sim_1 \reg (a)$, 
    %\item $\langle a, b \rangle \in \: \leq_t \circ \leq_k$ \: iff \:
    %  $\langle \reg(a), \reg(b) \rangle \in \: \leq_t \circ \leq_k$ \:
    %  iff \: $\reg(a) = \reg(a) \otimes \reg(b)$  \: iff \: $\reg(a) \leq_k \reg(b)$,
    \item $\langle a, b \rangle \in \: \leq_t \circ \leq_k$ \: iff \:
      $\langle \reg(a), \reg(b) \rangle \in \: \leq_t \circ \leq_k$ \: iff \: $\reg(a) \leq_k \reg(b)$,
    \item $a \sim_1 b$ \: iff \: $\reg(a) = \reg(b)$,
    %\item if $a \leq_k b$ then $\reg(a) \leq_k \reg(b)$. 
    \item $\reg (a \otimes b) = \reg (\reg(a) \otimes \reg(b)) = \reg(a) \otimes \reg(b) = \reg (a \land b)$,
    \item $\reg (a \oplus b) = \reg (\reg(a) \oplus \reg(b)) = \reg(a)
      \oplus \reg(b) = \reg (a \lor b)$.
  \end{enumerate}
    \end{proposition}
   
   \begin{proof}
(i). It is easy to check that if $a \in \Reg(\Al[B])$, then $a = \reg(a)$. The converse is immediate since, as we have observed,  $\reg(a)$ is always a regular element. Finally, if $a = \reg(b)$ for some $b \in B$, then  $a \in \Reg(\Al[B])$, which implies $a = \reg(a)$.

(ii). Note that, since $\Al[B]$ is interlaced, we have ${a \lor b} \sim_1 {a \oplus b}$ for all $a, b \in B$. Then
\begin{center}
  $\reg (a) \sim_1 a \lor (a \otimes \neg a) \lor \neg (a \lor (a \otimes
  \neg a)) = a \lor (a \otimes \neg a) \lor (\neg a \land (a \otimes
  \neg a)) =$ \\ 
  $a \lor (a \otimes \neg a) \sim_1 a \oplus (a \otimes \neg
  a) = a$.
  \end{center}
 
 (iii). The first equivalence follows immediately from the previous item and the transitivity of the relation $ \leq_t \circ \leq_k$. As to the second one, note that, by Proposition \ref{fileq} (i), we have $\langle a, b \rangle \in \: \leq_t \circ \leq_k$ iff $a \leq_{t} a \otimes b$. Now, if $a, b \in \Reg(\Al[B])$, then  $a \leq_{t} a \otimes b$ implies $\neg a \leq_{t} \neg  a \otimes \neg  b$, so by De Morgan's laws we obtain $a = a \otimes b$. The converse is easy, since by the interlacing conditions $a \leq_{k} b$ implies $a \leq_{k} a \land b$ and this, again  by Proposition \ref{fileq} (i), is equivalent to $\langle a, b \rangle \in \: \leq_t \circ \leq_k$.

(iv).  By (ii) and the transitivity of  $\sim_1$ it follows that $a \sim_1 b$ if and only if $\reg(a) \sim_1 \reg(b)$. To conclude the proof it is enough to note that, by (iii), we have $\reg(a) \sim_1 \reg(b)$ if and only if $\reg(a) = \reg(b)$. 

(v). By (ii) we have $a \sim_1 \reg(a)$ and $b \sim_1 \reg(b)$ for all $a, b \in B$. By Proposition \ref{prop:interlaced_pbl} (i), the relation $\sim_1$ is compatible with all bilattice operations except negation. Hence $a \otimes b \sim_1 \reg(a) \otimes \reg(b)$. By (iv) this implies $\reg (a \otimes b) = \reg (\reg(a) \otimes \reg(b))$. But  $\reg(a) \otimes \reg(b) \in \Reg(\Al[B])$, so we may apply (i) to obtain $ \reg (\reg(a) \otimes \reg(b)) =  \reg(a) \otimes \reg(b)$. Finally, the last equality is an easy consequence of (iv) together with Proposition \ref{prop:symetrization}.

(vi). Similar to the proof of (v).
\end{proof}
   
%   To prove property (ii) it is convenient to use that
%  \begin{center}
%  $\reg (a) \sim_1 a \lor (a \otimes \neg a) \lor \neg (a \lor (a \otimes
%  \neg a)) = a \lor (a \otimes \neg a) \lor (\neg a \land (a \otimes
%  \neg a)) =$ \\ 
%  $a \lor (a \otimes \neg a) \sim_1 a \oplus (a \otimes \neg
%  a) = a$.
%  \end{center}
  %$$
  %\reg (a) \sim_1 a \lor (a \otimes \neg a) \lor \neg (a \lor (a \otimes
  %\neg a)) = a \lor (a \otimes \neg a) \lor (\neg a \land (a \otimes
  %\neg a)) = \\ a \lor (a \otimes \neg a) \sim_1 a \oplus (a \otimes \neg
  %a) = a.
  %$$
  
%  It is now easy to prove the following:
%  
%  \begin{thm}
%\label{thm:rep_reg}
%Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus, \neg \rangle$ be an
%interlaced bilattice and $a \in B$. Then:
%%
%\begin{enumerate}[(i)]
%  \item $\Al[B] \cong \langle \Reg(\Al[B]), \otimes, \oplus \rangle
%  \odot \langle \Reg(\Al[B]), \otimes, \oplus \rangle.$
%  \item 

%  \end{enumerate}
%\end{thm}
  
  
  
  From the previous proposition it follows that
  the map $$\reg \!: \langle B, \otimes, \oplus \rangle \longrightarrow
  \langle \Reg(\Al[B]), \otimes, \oplus \rangle$$ is an epimorphism with
  kernel $\sim_1$. Therefore, $\langle B, \otimes, \oplus \rangle / \!\!
  \sim_1$ is isomorphic to $\langle \Reg(\Al[B]), \otimes, \oplus
  \rangle$. This suggests  that, as a different
  strategy to prove the Representation Theorem (Theorem \ref{thm:interlaced_bl}), we could have directly shown
  that $$\Al[B] \cong \langle \Reg(\Al[B]), \otimes, \oplus \rangle
  \odot \langle \Reg(\Al[B]), \otimes, \oplus \rangle.$$
It is not difficult to check that the isomorphism is given by the map $f: B \longrightarrow \Reg(\Al[B]) \times \Reg(\Al[B])$ defined, for all $a \in B$, as $$f(a) = \la \reg(a), \reg(\neg a) \ra.$$ Its inverse $f^{-1} :  \Reg(\Al[B])  \times \Reg(\Al[B]) \longrightarrow B $ is defined,  for all $a, b \in \Reg(\Al[B])  $, as 
$$f^{-1} (\la a, b \ra) = (a \otimes (a \lor b)) \oplus (b \otimes (a \land b)).$$ 
Notice that this implies that  $\Al[B]$ is generated by the set $\Reg(\Al[B]) $, for we have, for any $a \in B$, $$a = (\reg(a) \otimes (\reg(a) \lor \reg(\neg a))) \oplus (\reg(\neg a) \otimes (\reg(a) \land \reg(\neg a))).$$




To end the section, we state an analogue of
Theorem~\ref{thm:representation_eq} for
bilattices:

%\texttt{Por lo que respecta a (1), (2) y (3) no se generaliza nada. Todo bilattice tiene como reducto un pre-bilattice y  las ecuaciones que consideras no usan negacion. Por tanto (1) (2) y (3) se siguen del teorema \ref{thm:representation_eq} } 

\begin{thm}
  \label{thm:representation_bl_eq}
  Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus , \neg \rangle$ be a bilattice and let $\varepsilon(\sqcap,\sqcup)$ be an
  equation in the language of lattices. The following statements are
  equivalent.
  \begin{enumerate}
    \item $\Al[B]$ is interlaced and $\Al[B]
      \models \{ \varepsilon(\land,\lor), \varepsilon(\lor,\land)
      ,\varepsilon(\otimes,\oplus),  \varepsilon(\oplus,\otimes) \}$.
    \item $\Al[B]$ is interlaced and  $\Al[B]
      \models \{ \varepsilon(\land,\lor), \varepsilon(\lor,\land) \}$.
    \item $\Al[B]$ is interlaced and  $\Al[B]
      \models \{ \varepsilon(\otimes,\oplus), \varepsilon(\oplus,\otimes) \}$.
    \item There is a lattice $\Al[L]$ such that
      $\Al[L] \models \{ \varepsilon(\sqcap,\sqcup),
      \varepsilon(\sqcup, \sqcap) \}$ and
      $\Al[B]$ is isomorphic to $\Al[L] \odot \Al[L]$.
  \end{enumerate}
\end{thm}

\begin{proof}
  Essentially the same as that of Theorem~\ref{thm:representation_eq},
except that now  we use Theorem~\ref{thm:interlaced_bl}.
\end{proof}






\section{Bifilters}
\label{sec:bif}

As in lattice theory, an important topic in (pre-)bilattice theory is the study of filters and ideals. Some results on this subject have already been obtained in \cite{Ko01a}
for the case of bounded (pre-)bilattices. In this section we complete this study  for the case of (unbounded) interlaced and distributive (pre-)bilattices, also  establishing some connections with what was done in Section~\ref{sec:reppre}.

%has not been investigated in the literature, not even in the case of bounded (pre-)bilattices. In this section we try to fill this gap for the case of interlaced and distributive (pre-)bilattices, also  establishing some connections with what was done in Section~\ref{sec:reppre}.

Since (pre-)bilattices have two orders, the notions of filter and ideal in lattices can be naturally translated in four possible ways: we can consider subsets that are filters of both orders, filters of one and ideals of the other, etc. Of this four, the only notion that has been considered in the literature so far is that of ``bifilter'', introduced by Arieli and Avron (see, for instance, \cite{ArAv96}) through the following:

\begin{definition} \label{def:bifilter}
A \emph{bifilter} of a (pre-)bilattice $\Al[B] = \left\langle B, \land,
\lor, \otimes, \oplus \right\rangle$  is  a non-empty set
$F \subseteq B$ such that $F$ is a lattice filter of both orders $\leq_t$ and
$\leq_k$. A bifilter $F$ is \emph{prime} if $a \lor b \in F$ implies $a \in F$ or $b \in F$ and $a \oplus b \in F$ implies $a \in F$ or $b \in F$  for all $a,b \in B$.
\end{definition} 

Since the family $\{ \emptyset \} \cup \{ F \subseteq B: F
\textrm{ is a bifilter of } \Al[B] \}$ is closed under arbitrary intersections, it forms a closure system: we can then consider its associated closure operator, which we will denote by $\FF$. 

Note that, if $\Al[B]$ is bounded, then it is not necessary to include the empty set in the previous family, because then the bifilter generated by $\true$ (or, equivalently, by $\top$) is included in all bifilters: hence %, in a bounded pre-bilattice, 
the intersection of any family of bifilters is non empty. However, this is not true in general for unbounded pre-bilattices, so if we did not add the empty set to the family of all bifilters, we could not guarantee that $\FF$ is indeed a closure operator.

 It
holds that $\FF(\emptyset) = \emptyset$ and that if
$X \neq \emptyset$, then $\FF(X)$ is  exactly the smallest bifilter containing $X$. This is a consequence of the fact that if $X \neq \emptyset$, then
$\emptyset \neq \bigcap \{ F \subseteq B:  F
\textrm{ is a bifilter of } \Al[B] \textrm{ such that } X \subseteq F
\}$. This claim can be easily checked using that if $a \in X$ then the
set $\{ x \in B: a \leq_k a \land x \}$, which is considered below, is a
subset of $\bigcap \{ F \subseteq B:  F \textrm{ is a bifilter of }
\Al[B] \textrm{ such that } X \subseteq F \}$.  

As usual, we write
$\FF (a)$ as an abbreviation for $\FF(\{a\})$. 

As we have anticipated, one could consider the other three possible closure operators: $\II$ (ideal in both orders, which we may call \emph{biideal}), $\FI$ (filter in
the truth order and ideal in the knowledge order) and $\IF$ (ideal in
the truth order and filter in the knowledge order). However, it is enough to consider the bifilter operator only, because by the Duality Principle we have that on any interlaced pre-bilattice  $\langle B, \leq_t, \leq_k\rangle$
\begin{itemize}
  \item $\II$ coincides with the
    operator $\FF$ over  $\langle B, \geq_t, \geq_k\rangle$
  \item $\FI$ coincides with the
    operator $\FF$ over  $\langle B, \leq_t, \geq_k\rangle$
  \item $\IF$ coincides with the
    operator $\FF$ over $\langle B, \geq_t, \leq_k\rangle$.
\end{itemize}

%\texttt{La notacion me parece que puede inducir a confusion. ¿No seria mejor usar los ordenes? Dado $\langle B, \land, \lor, \otimes, \oplus\rangle$, lo que se considera es $\langle B, \geq_t, \geq_k\rangle$, $\langle B, \leq_t, \geq_k\rangle$
%y $\langle B, \geq_t, \leq_k\rangle$.}

%The following lemma provides a characterization of the bifilter generated by a set:

%\begin{lem}
%  \label{lem:bifilter}
%  Let $\Al[B]$ be an interlaced (pre-)bilattice and let $X$ be a
%  subset of $B$. Then,
%   $$\FF (X) \: = \: (\leq_t \circ \leq_k) [X] \: = \: (\leq_k \circ
%   \leq_t ) [X].$$
%\end{lem} 

%\begin{proof}
%  If $X$ is empty it is trivial, so let us suppose that it is not.
%  By duality it is enough to prove that $\FF (X) \: = \: (\leq_t \circ
%  \leq_k) [X]$. Hence, it suffices to prove that $(\leq_t \circ
%  \leq_k) [X]$ is a bifilter of $\Al[B]$, and this is a trivial consequence
%  of Corollary~\ref{cor:interlacingorders}.
%  
%  \texttt{Estas seguro? ¿ Por que $(\leq_t \circ
%  \leq_k) [X]$ est\'a cerrado bajo $\wedge$, por ejemplo?} 
%  XXX
%\end{proof}

The following lemma provides a characterization of the bifilter generated by a set. Let us use the following abbreviations: $\bar{a} = a_{1}, \ldots, a_{n} $ for some $n > 0$, $\land (\bar{a}) = a_{1} \land \ldots \land a_{n} $ and $\otimes (\bar{a}) = a_{1} \otimes \ldots \otimes a_{n} $.


\begin{lem} \label{lem:bifilter} 
Let $\Al[B]$ be an interlaced (pre-)bilattice and let $X$ be a subset of $B$. Then 
%
\begin{align*}
   \FF (X)  & =  \{ a \in B : \exists \ \bar{a} \in X \textrm{ s.t. } \la \land (\bar{a}), a \ra \in  {\leq_t \circ \leq_k}  \} \\
    &   =  \{ a \in B : \exists \ \bar{a} \in X \textrm{ s.t. } \la \otimes (\bar{a}), a \ra \in  {\leq_t \circ \leq_k}  \}.  
\end{align*} 
%
%%
%\begin{align*}
%   \FF (X)  & =  \{ a \in B : \exists \ a_{1}, \ldots, a_{n} \in X \textrm{ s.t. } \la a_{1} \land \ldots \land a_{n}, a \ra \in  {\leq_t \circ \leq_k}    \textrm{ for some } n > 0 \} \\
%    &   =  \{ a \in B : \exists \ a_{1}, \ldots, a_{n} \in X \textrm{ s.t. } \la a_{1} \otimes \ldots \otimes a_{n}, a \ra \in  {\leq_t \circ \leq_k} \textrm{ for some } n > 0  \}.  
%\end{align*} 
\end{lem} 

\begin{proof}
  If $X$ is empty it is trivial, so suppose it is not and let 
  $$F = \{ a \in B : \exists \ \bar{a} \in X \textrm{ s.t. } \la \land (\bar{a}), a \ra \in  {\leq_t \circ \leq_k}  \}. $$
  %$$F = \{ a \in B : \exists \ a_{1}, \ldots, a_{n} \in X \textrm{ s.t. } \la a_{1} \land \ldots \land a_{n}, a \ra \in  {\leq_t \circ \leq_k}    \textrm{ for some } n > 0 \}. $$
%
Using Proposition~\ref{fileq} (i) and Corollary~\ref{cor:interlacingorders}, it is not difficult to prove that
%
\begin{equation}
\label{e:bif}
F =   \{ a \in B : \exists \ \bar{a} \in X \textrm{ s.t. } \la \otimes (\bar{a}), a \ra \in  {\leq_t \circ \leq_k}  \}.
\end{equation}
%
%$$
%F =  \{ a \in B : \exists \ a_{1}, \ldots, a_{n} \in X \textrm{ s.t. } \la a_{1} \otimes \ldots \otimes a_{n}, a \ra \in  {\leq_t \circ \leq_k} \textrm{ for some } n > 0  \}.  
%$$
In fact, if $\la a_{1} \land \ldots \land a_{n}, a \ra \in  {\leq_t \circ \leq_k}$, then  $\la a_{1} \land \ldots \land a_{n}, a \ra \in  {\leq_k \circ \leq_t}$. By the interlacing conditions $  a_{1} \otimes \ldots \otimes a_{n} \leq_{k} a_{1} \land \ldots \land a_{n}$, so  $\la a_{1} \otimes \ldots \otimes a_{n}, a \ra \in  {\leq_k \circ \leq_t}$, which is equivalent to $\la a_{1} \otimes \ldots \otimes a_{n}, a \ra \in  {\leq_t \circ \leq_k}$. By symmetry we have that $\la a_{1} \otimes \ldots \otimes a_{n}, a \ra \in  {\leq_t \circ \leq_k}$ implies $\la a_{1} \land \ldots \land a_{n}, a \ra \in  {\leq_t \circ \leq_k}$, so the two conditions are equivalent.

 
Now, to see that $F \subseteq \FF (X) $, assume $a \in F$. This means that there are $a_{1}, \ldots, a_{n} \in X$ and $b \in B$ such that $a_{1} \land \ldots \land a_{n} \leq_{t} b \leq_{k} a$. Since $\FF (X) $ is closed under $\land$, we have $a_{1} \land \ldots \land a_{n} \in \FF (X)$, and since it is upward closed w.r.t.\ both lattice orderings, we have $ a, b \in \FF (X)$ as well. 

Clearly  $X \subseteq F$. Hence, in order to prove that $\FF (X) \subseteq F $, it is sufficient to check that $F$ is a bifilter. That $F$ is closed under $\land$ follows immediately from the interlacing conditions; to show that it is closed under $\otimes$ we can use what we have proved in (\ref{e:bif}) above. 
%$$
%F =  \{ a \in B : \exists \ a_{1}, \ldots, a_{n} \in X \textrm{ s.t. } \la a_{1} \otimes \ldots \otimes a_{n}, a \ra \in  {\leq_t \circ \leq_k} \textrm{ for some } n > 0  \}.  
%$$ 
Finally, that $F$ is upward closed w.r.t.\ both orders is also an immediate consequence of Corollary~\ref{cor:interlacingorders}. 
% 
%  By duality it is enough to prove that $\FF (X) \: = \: (\leq_t \circ
%  \leq_k) [X]$. Hence, it suffices to prove that $(\leq_t \circ
%  \leq_k) [X]$ is a bifilter of $\Al[B]$, and this is a trivial consequence
%  of Corollary~\ref{cor:interlacingorders}.
%  
\end{proof}

  
%\texttt{Estas seguro? ¿ Por que $(\leq_t \circ \leq_k) [X]$ est\'a cerrado bajo $\wedge$, por ejemplo?} 
   
%\texttt{Umberto: Creo que el lema \ref{lem:bifilter} estaba mal: lo he cambiado, junto col la prueba, y creo que ahora est\'{a} bien.} 
 


Thus, by the first item of Proposition~\ref{fileq} it is straightforward to prove the following:

\begin{cor} 
  \label{cor:bifilters}
  Let    $\Al[B] = \langle B, \land, \lor, \otimes, \oplus\rangle$ be an interlaced pre-bilattice. Then, for
every $X \cup \{ a,b \} \subseteq B$:
\begin{enumerate}[(i)]
    \item $\FF (a) = \{ x \in B: a \leq_k a \land x \} \ \! \! = \{ x \in B: a
        \leq_t a \otimes x \} \\  \textrm{ } \quad \quad \; \; \ \! \! = \{ x \in B: a \lor x \leq_k x \} = \{ x \in
   B: a \oplus x \leq_t x \}$,
  \item $a \sim_1 b$ \quad iff \quad $\FF(a) = \FF(b)$,
  \item $\FF (a \lor b) = \FF(a) \cap \FF(b) = \FF (a \oplus b)$,
  \item $\FF (a \land b) = \FF(a) \lor \FF(b) = \FF (a \otimes b)$,
  \item $\FF (X) = \{ x \in B:  \exists \ \bar{a} \in X \textrm{ s.t. } \land (\bar{a}) \leq_k \land (\bar{a}) \land x \} \\ 
 \textrm{ } \quad \quad \ \ \!   \: \,   =  \{ x \in B:  \exists \ \bar{a} \in X \textrm{ s.t. } (\land (\bar{a}) ) \lor
    x \leq_k x  \} 
    \\  \textrm{ } \quad \quad \ \ \!   \: \,  = \{ x \in B:  \exists \ \bar{a} \in X \textrm{ s.t. } \otimes  (\bar{a})  \leq_t \otimes  (\bar{a})  \otimes x  \}  \\ 
    \textrm{ } \quad \quad \ \ \!   \: \,   =  \{ x \in B:  \exists \ \bar{a} \in X \textrm{ s.t. } (\otimes  (\bar{a}))
    \oplus x \leq_t x \}.$
    %\item If $\Al[B] $ is distributive, then $F(X, a \lor b) = F(X, a \oplus b) = F(X, a) \cap F(X, b)$. 
\end{enumerate}
\end{cor} 

%\begin{proof}
%(vi). Since $a \lor b \in F(X, a)$ and $a \lor b \in F(X, b)$, it is clear that $F(X, a \lor b) \subseteq F(X, a) \cap F(X, b)$. For the other inclusion, suppose that $c \in F(X, a)$ and $c \in F(X, b)$. Then there are $a_1 \ldots  a_n, b_1 \ldots  b_m \in X$ such that $ a_1 \otimes \ldots \otimes a_n \otimes a \leq_k (a_1 \otimes \ldots \otimes a_n \otimes a) \land c $ and $b_1 \otimes \ldots \otimes b_m \otimes b \leq_k (b_1 \otimes \ldots \otimes b_m \otimes b) \land c$. Let $d = a_1 \otimes \ldots \otimes a_n \otimes b_1 \otimes \ldots \otimes b_m $. Then $d \otimes a \leq_k  (a_1 \otimes \ldots \otimes a_n \otimes a) \land c \leq_t c$ and $d \otimes b \leq_k (b_1 \otimes \ldots \otimes b_m \otimes b) \land c \leq_t c$. Using the interlacing conditions and distributivity we have $ (d \otimes a) \lor (d \otimes b) = d \otimes (a \lor b) \leq_k ((a_1 \otimes \ldots \otimes a_n \otimes a) \land c) \lor ((b_1 \otimes \ldots \otimes b_m \otimes b) \land c) \leq_t c$. Therefore $d \otimes (a \lor b) \otimes  (((a_1 \otimes \ldots \otimes a_n \otimes a) \land c) \lor ((b_1 \otimes \ldots \otimes b_m \otimes b) \land c)) = d \otimes (a \lor b) \leq_t d \otimes (a \lor b) \otimes c $. Hence  $c \in F(X, a \lor b)$, i.e. $F(X, a) \cap F(X, b) \subseteq F(X, a \lor b)$.
%\end{proof}



In particular, we may now recognize that the congruence relation $\sim_1$ introduced in
Section~\ref{sec:reppre} is the one induced by the principal
bifilters. Using the other three items from Proposition~\ref{fileq} we
would get similar characterizations of $\IF$, $\FI$ and $\II$. 
%indeed $\IF = (\geq_t \circ \leq_k)$, $\FI = (\leq_t \circ \geq_k)$ and $\II = (\geq_t \circ \geq_k)$. 
We point out that,
for every $a, b \in B$,
%\begin{center}
%  $a \sim_1 b$ \quad iff \quad $\FF(a) = \FF(b)$ \quad iff \quad $\II(a)
%  = \II(b)$,
%\end{center}
%%and
%\begin{center}
%  $a \sim_2 b$ \quad iff \quad $\FI(a) = \FI(b)$ \quad iff \quad $\IF(a)
%  = \IF(b)$.
%\end{center}

\begin{center}
\begin{tabular}{cccccccccc}

 $a  \sim_1 b$ & & iff & & $ \FF(a) = \FF(b)$ & & iff && $ \II(a)  = \II(b)$ \\
 $a  \sim_2 b$ & & iff & & $\FI(a)  = \FI(b)$  &  & iff && $\IF(a)  = \IF(b)$.  
\\
\end{tabular}
\end{center}

It is also worth noting that in the case that $\Al[B]$ is a
bilattice (i.e., there is a negation operation) we can characterize principal bifilters as follows:
$$\FF(a) = \{ x \in B: \reg (a) \leq_k \reg(x) \}.$$ 
This result follows easily from Corollary \ref{cor:bifilters} (i) and Proposition \ref{prop:regular} (iii).
%\texttt{No deberias dar la demostracion?}
Moreover, we have that
\begin{align*}
\IF(a) & = \{ x \in B: \neg x \in \FF(\neg a) \} \\
\FI(a) & = \{ x \in B: \neg a \in \FF(\neg x) \} \\
\II(a) & = \{ x \in B: a \in \FF (x) \}.
\end{align*}

Note that, in fact, negation does not play any
role in the last characterization of $\II(a)$,  hence the result also holds in pre-bilattices; we have written it here only for the
sake of completeness.

To finish this section, we study the relationship between the bifilters of the interlaced pre-bilattice
$\Al[L_1] \odot \Al[L_2]$ and the lattice filters of the lattices $\Al[L_1]$ and
$\Al[L_2]$.


\begin{proposition} \label{prop:bifilprod}
Let $\Al[L_1] \odot \Al[L_2]$ be a product (pre-)bilattice,
%$\Al[B] = \langle B, \land, \lor, \otimes, \oplus \rangle$  be the interlaced pre-bilattice $\Al[L_1] \odot \Al[L_2]$ for some lattices
where $\Al[L_1] = \la L_{1}, \sqcap_{1},$ $\sqcup_{1}  \ra$ and $\Al[L_2] = \la L_{2}, \sqcap_{2}, \sqcup_{2}  \ra$. If $F $
is a nonempty subset of $L_{1} \times L_{2}$, then
  \begin{enumerate}[(i)]
    \item  $F$ is a bifilter of $\Al[L_1] \odot \Al[L_2]$  iff  $ \; F=
      \overline{F} \times L_2 $ for some lattice filter $\overline{F}$ of $\Al[L_1]$.
    \item  $F$ is a prime bifilter of $\Al[L_1] \odot \Al[L_2]$ iff $\; F=
      \overline{F} \times L_2 $ for some prime filter $\overline{F}$ of $\Al[L_1]$.
\end{enumerate}
\end{proposition}

%\texttt{Hay demasiado espacio antes y despues de "if and only if".\\ ¿Hay alguna raz\'on para no usar "iff"?}

\begin{proof} 
(i). The leftwards implication is trivial. For the other direction, 
assume that $F$ is a bifilter of $\Al[L_1] \odot \Al[L_2]$. Since $\pi_1 [F]$ is
obviously a lattice filter, it suffices to prove that $F = \pi_1[F]
\times L_2$. The only non trivial inclusion to justify is that $\pi_1[F]
\times L_2 \subseteq F$. Hence, let us consider a pair $\langle a,b
\rangle \in \pi_1[F] \times L_2$. Since $a \in \pi_1 [F]$ we know that
there is some $c \in L_2$ such that $\langle a,c \rangle \in F$. Now,
using that
\begin{center}
  $\langle a,c \rangle \leq_t \langle a, b \sqcap_2 c \rangle \leq_k \langle a,b \rangle$
\end{center}
together with the closure properties of a bifilter we get that
$\langle a,b \rangle \in F$.

(ii). Again the leftwards direction is trivial; hence we consider a
prime bifilter $F$ of $\Al[L_1] \odot \Al[L_2]$ in order to prove the converse direction.
By the previous item in this result we know that $F = \pi_1[F] \times
L_2$. Thus, it suffices to prove that $\pi_1[F]$ is a prime lattice. Let
us consider a pair of elements $a,b \in L_1$ such that $a \sqcup_1 b \in
\pi_1[F]$. Then for all $c \in L_2$, it holds that $\langle a, c \rangle
\lor \langle b, c \rangle = \langle a \sqcup_1 b, c \rangle \in \pi_1[F]
\times L_2 = F$. Using that $L_2$ is non empty we get that $\langle a,
c \rangle \lor \langle b,c \rangle \in F$ for some $c \in L_2$. Since
$F$ is prime, this implies that either $\langle a, c \rangle \in F$ or
$\langle b, c \rangle \in F$. Therefore we have that either $a \in
\pi_1[F]$ or $b \in \pi_1[F]$.
\end{proof}

The previous result has an obvious dual which can be proved in the same way. Recall that a biideal of a bilattice is an ideal of both orders, and it is prime if it is a prime ideal of both the t- and the k-lattice. 

\begin{proposition} \label{prop:biidprod}
Let $\Al[L_1] \odot \Al[L_2]$ be a product (pre-)bilattice,
%$\Al[B] = \langle B, \land, \lor, \otimes, \oplus \rangle$  be the interlaced pre-bilattice $\Al[L_1] \odot \Al[L_2]$ for some lattices
where $\Al[L_1] = \la L_{1}, \sqcap_{1},$ $\sqcup_{1}  \ra$ and $\Al[L_2] = \la L_{2}, \sqcap_{2}, \sqcup_{2}  \ra$. If $I $
is a nonempty subset of $L_{1} \times L_{2}$, then
  \begin{enumerate}[(i)]
    \item  $I$ is a biideal of $\Al[L_1] \odot \Al[L_2]$  iff  $ \; I=
      \overline{I} \times L_2 $ for some lattice ideal $\overline{I}$ of $\Al[L_1]$.
    \item  $I$ is a prime biideal of $\Al[L_1] \odot \Al[L_2]$ iff $\; I=
      \overline{I} \times L_2 $ for some prime ideal $\overline{I}$ of $\Al[L_1]$.
\end{enumerate}
\end{proposition}

\begin{rem}
\label{r:filt}
An interesting consequence of the previous propositions is that the lattice of bifilters (biideals) of an interlaced pre-bilattice  $\Al[L_1] \odot \Al[L_2]$ is isomorphic to the lattice of filters (ideals) of the first factor lattice $\Al[L_1]$ (note that the second factor $\Al[L_2]$ does not play any role here). So, for instance, if $\Al[L_1]$ is distributive (hence the lattice of its filters is distributive), then the lattice of bifilters of $\Al[L_1] \odot \Al[L_2]$ is also distributive. This result applies, in particular, to the class of distributive (pre-)bilattices, which is the subject of the following section.
\end{rem}

 



\section{The variety of distributive (pre-)bilattices}
\label{sec:dis}

In this section we shall focus on distributive (pre-)bilattices. First of all, let us recall some known facts. 

An immediate consequence of the results of \cite{MoPiSlVo00}, although not explicitly stated there (nor anywhere else in the literature on bilattices), is that the variety of bounded distributive bilattices is generated by $\four$, and that  the variety of bounded distributive pre-bilattices is generated by its two-element member. The proof of these results is based on the Representation Theorem for bounded bilattices together with the fact that the two-element lattice generates
the variety of bounded distributive lattices. 

Having extended the Representation Theorem
to the unbounded case, we can now easily obtain the corresponding results for unbounded (pre-)bilattices. Using Propositions  \ref{prop:interlaced_pbl} and \ref{prop:interbl_cong} together with Theorem \ref{thm:interlaced_bl}, we immediately have the following:

\begin{thm} 
\
  \begin{itemize}
%    \item The variety $\DPBL$ has only one subdirectly irreducible
%      algebra, which  is its two-element member.
\item The variety $\DPBL$ has two subdirectly irreducible algebras, i.e.\ the two two-element pre-bilattices
    whose direct product is the pre-bilattice  $\four$.
    %\item The variety $\DPBL$ is generated by its two element member.
       \item The variety $\DPBL$ is generated by its two two-element members.
    \item The variety $\DBL$ has only one subdirectly irreducible
      algebra, which is $\four$.
    \item The variety $\DBL$ is generated by $\four$.
  \end{itemize}
\end{thm}

It is not difficult to see that the previous theorem also implies that the variety $\DBL$ has no proper sub-quasivarieties (see also Lemma \ref{l:submat}). In the remaining part of the section we shall prove some results on distributive pre-bilattices that can be regarded as analogues of  well-known properties of distributive lattices.

\begin{proposition}
  \label{prop:bifil_dbl}
  Let $\Al[B]$ be a distributive (pre-)bilattice. Then, for every set
  $X \cup \{ a, b \} \subseteq B$, it holds that
  $$
  \FF (X,a \lor b) = \FF(X,a) \cap \FF(X,b) = \FF (X,a \oplus b).
  $$
\end{proposition} 

\begin{proof}
  By duality it is enough to prove that $\FF (X,a \lor b) = \FF(X,a)
  \cap \FF(X,b)$. The inclusion $\FF (X,a \lor b) \subseteq \FF(X,a) \cap
  \FF(X,b)$ is trivial, and next we prove the other inclusion. To this
  purpose let us assume that $c \in A$ is such that $c \in \FF(X,a)$ and
  $c \in \FF(X,b)$. Hence, there are some $a_1, \ldots, a_n \in X$ such
  that $c \in \FF (a_1 \land \ldots \land a_n \land a)$ and $c \in
  \FF (a_1 \land \ldots \land a_n \land b)$. Thus, $\langle a_1 \land
  \ldots \land a_n \land a, c \rangle \in \: \leq_t \circ \leq_k$ and $\langle a_1 \land
  \ldots \land a_n \land b, c \rangle \in \: \leq_t \circ \leq_k$. Using
  that $\leq_t \circ \leq_k$ is a quasi order compatible with the
  operations it follows that $\langle a_1 \land
  \ldots \land a_n \land (a \lor b), c \rangle = \langle (a_1 \land
  \ldots \land a_n \land a) \lor (a_1 \land
  \ldots \land a_n \land b), c \lor c \rangle \in \: \leq_t \circ
  \leq_k$. Therefore, $c \in \FF (a_1 \land \ldots \land a_n \land (a
  \lor b) )$; and so $c \in \FF (X, a \lor b)$.
\end{proof}

%\texttt{Esta propiedad implica que el reticulo de los bifiltros es distributivo. Quizas vale la pena decirlo.}
%\texttt{Umberto: En vez de decir aqu\'{i} que esta propiedad implica que el ret\'{i}culo de los bifiltros es distributivo, he puesto en el \'{u}ltimo p\'{a}rrafo de la Section \ref{sec:bif} un resultado algo m\'{a}s general, que lo implica.}


%We shall now focus on distributive pre-bilattices in order to prove some results that are in some sense analogue to well-known properties of distributive lattices.

 Using  Proposition \ref{prop:bifilprod}, we may prove a kind of Prime Bifilter Theorem for distributive (pre-)bilattices:

\begin{proposition} \label{primebif2} 
Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus \rangle$ be a distributive pre-bilattice. Let $F$ be
a non-empty proper bifilter and $I$ a biideal %(i.e., an ideal of both the t-lattice and the k-lattice) 
of $\Al[B]$  such that $F \cap I = \emptyset $. Then there exists a
prime bifilter $P$ of $\Al[B]$ such that $F \subseteq P$ and $P \cap I = \emptyset $.
\end{proposition}

\begin{proof}
By the previous results we may assume that $\Al[B] \cong \Al[L_1] \odot \Al[L_2]$ for some distributive lattices $\langle L_1, \sqcap_1, \sqcup_2 \rangle$ and $\langle L_2, \sqcap_2, \sqcup_2 \rangle$. Moreover, we know that $F = F_1 \times L_2$ and $I = I_1 \times L_2$, where $F_1 \subseteq L_1$ is a lattice filter and $I_1 \subseteq L_1$ is a lattice ideal. Since $L_1$ is distributive, by the Prime Filter Theorem we know that there is a prime filter $P_1 \subseteq L_1 $ such that $F_1 \subseteq P_1$ and $P_1 \cap I_1 = \emptyset $. We claim that $P = P_1 \times L_2$ is the desired prime bifilter. Clearly $F \subseteq P$, and by the previous results we know that $P$ is a prime bifilter. Moreover, if there were $\langle a, b \rangle \in P \cap I$, then we would have $a \in P_1 \cap I_1$, against the hypothesis. Hence $P \cap I = \emptyset $ and we are done.
\end{proof}

Using Proposition \ref{primebif2}, it is easy to prove the following bifilter extension property:

\begin{proposition} \label{bifext}
Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus \rangle$ be a distributive pre-bilattice. Let $F$ be
a non-empty proper bifilter. Then there is a prime bifilter $P \subseteq B$ such that $F \subseteq P \varsubsetneq B$. 
\end{proposition}

\begin{proof}
Assume $F \in B$ is a proper bifilter, i.e there is $a \in B$ s.t. $a \notin F$. Let $I = \II(a)$. Note that $F \cap I = \emptyset $. Indeed, if there were some $b \in F \cap I$, then by the
former condition we would have $\FF(b) \subseteq F$, and by the latter we would have $ a \oplus b \leq_t a$. Since $b \leq_k a \oplus b \leq_t a$, this implies that $a \in \FF(b) \subseteq F $, against the assumption. Hence  $F \cap I = \emptyset $. Now we can apply Proposition \ref{primebif2} and the result easily follows.  
\end{proof}

%\texttt{No hablaria de que un reticulo o un (pre-)bireticulo tiene el Prime Bifilter Theorem. El Prime Bifilter Theorem tiene una cuantificaci\'on sobre todo (pre-) bireticulo distributivo. Adem\'as, un teroema es un enunciado y no tiene sentido decir que un objeto tiene un enunciado. Hablaria de la Prime bifilter property}

It is known that for lattices the Prime Filter Theorem is equivalent to distributivity. Hence, using Proposition \ref{primebif2}, it is possible to prove that an interlaced pre-bilattice $ \Al[L_1]  \odot \Al[L_2]$ has the prime bifilter property stated in Proposition \ref{primebif2}  if and only if $\Al[L_1]$ is a distributive lattice. In fact, recalling Propositions \ref{prop:bifilprod} and \ref{prop:biidprod}, it is easy to see that if $ \Al[L_1]  \odot \Al[L_2]$ has the prime bifilter property, then $ \Al[L_1]$ has the prime filter property, hence is distributive; the converse is also easy. However, it is not true that if a pre-bilattice has the prime bifilter property then it is distributive: for a counterexample we just need to consider any pre-bilattice $\Al[L_1]  \odot \Al[L_2]$ where $\Al[L_1]$ is a distribuitve lattice while $\Al[L_2]$ is not distributive. 

Note also that it is not true that given a pre-bilattice $\Al[B]$ and $a, b \in B$, if $a \neq b$ then there is a bifilter $F$ such that $a \in F$ and $b \notin F$. For instance, we have that $ \top \in F$ iff $t \in F$, for every bifilter $F$. This is so because $t \leq_k \top$ and $\top \leq_t t$, so $t \in F$ implies $\top \in F$ and conversely. However, it is possible to prove the following:

\begin{proposition} \label{bifsep}
Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus \rangle$ be a distributive pre-bilattice and $a, b \in B$ s.t. $a \neq b$. Then either there is a prime bifilter $F \subset B$ such that $a \in F$ and $b \notin F$ or there is a prime t-ideal and k-filter $I \subset B$ such that $a \in I$ and $b \notin I$. 
\end{proposition}

\begin{proof}
From the preceding results we know that if $\FF(a) = \FF (b)$ and $\II(a) = \II (b)$, then $a=b$. By contraposition, we have that $a \neq b$ implies that either $\FF(a) \neq \FF (b)$ or $\II(a) \neq \II (b)$. Assume the first. By the Prime Bifilter Theorem we know that $\FF(a)$ and $\FF(b)$ are intersections of a family of prime bifilters, so there must be some prime bifilter $G$ in the family that is not in the other. So we have, for instance, $a \in G$ but $b \notin G$. Assuming the second, by the same reasoning we may conclude that there is a prime t-ideal and k-filter $H$ such that $a \in H$ but $b \notin H$.
\end{proof}


%\texttt{Yo no formularia el resultado que viene a continuaci\'on como has hecho. Lo que demuestras es que todo (pre-)bilattice distributivo es isomorfo a un producto de reticulos de conjuntos. Esto se sigue del teorema de representacion y del hecho de que todo reticulo distributivo es isomorfo a un reticulo de de conjuntos. Yo pondria el enfasis en la construccion particular con bifiltros y t,k ideal-filtros que lleva al resultado.} 

Using the previous result, we can state a representation theorem for distributive bilattices analogous to the one we have for distributive lattices. Let us denote by $Pr \FF (\Al[B]) $ the family of prime bifilters of a (pre-)bilattice $\Al[B]$ and by  $Pr \IF (\Al[B]) $ the family of prime t-ideal and k-filters of $\Al[B]$. Then we have the following:

\begin{proposition}
Every distributive (pre-)bilattice $\Al[B]$  is isomorphic to a sub\-(pre-)\-bilattice of  the (pre-)bilattice of sets:
$$\langle P( Pr \FF (\Al[B]) ), \cap, \cup \rangle \odot \langle P( Pr \IF (\Al[B]) ), \cap, \cup \rangle $$   
through the mapping $\sigma$, defined, for all $a \in B$, as $\sigma (a) = \langle \sigma^+(a), \sigma^-(a) \rangle$, where
\begin{align*}
\sigma^+(a) & = \{X \subseteq B : X \textrm{ is a prime bifilter and } a \in X \}; \\
\sigma^-(a) & = \{Y \subseteq B : Y \textrm{ is a prime t-ideal and k-filter and } a \in Y \}.
\end{align*}
If  $\Al[B]$ has a negation, then the map $\sigma^-$ may also be defined as
$$
\sigma^-(a)  = \{ X \subseteq B : X \textrm{ is a prime bifilter and } \neg a \in X \}.
$$
\end{proposition}

\begin{proof}
%The mapping is defined as follows. For $a \in B$, let $\sigma (a) = \langle \sigma^+(a), \sigma^-(a) \rangle$, where
%\begin{align*}
%\sigma^+(a) & = \{P \subseteq B : P \textrm{ is a prime bifilter and } a \in P \}; \\
%\sigma^-(a) & = \{R \subseteq B : R \textrm{ is a prime t-ideal and k-filter and } a \in R \}.
%\end{align*}
Note that we have:
 
\begin{enumerate}[(i)]
\item $\sigma(a \land b)  = \langle \sigma^+(a) \cap \sigma^+(b), \sigma^-(a) \cup \sigma^-(b) \rangle$
\item  $\sigma(a \lor b)  = \langle \sigma^+(a) \cup \sigma^+(b), \sigma^-(a) \cap \sigma^-(b) \rangle$
\item $\sigma(a \otimes b)  = \langle \sigma^+(a) \cap \sigma^+(b), \sigma^-(a) \cap \sigma^-(b) \rangle$
\item $\sigma(a \oplus b)  = \langle \sigma^+(a) \cup \sigma^+(b), \sigma^-(a) \cup \sigma^-(b) \rangle$.
\end{enumerate}

(i). Follows from the fact that, for any bifilter $F$, we have $a \land b \in F$ iff $a, b \in F$ and, for any prime t-ideal and k-filter $I$, we have $a \land b \in I$ iff $a \in I$ or $b \in I$.

(ii). Follows from the fact that, for any prime bifilter $F$, we have $a \lor b \in F$ iff $a \in F$ or $b \in F$ and, for any t-ideal and k-filter $I$, we have $a \lor b \in I$ iff $a, b \in I$.

(iii). Follows from the fact that, for any bifilter $F$, we have $a \otimes b \in F$ iff $a, b \in F$ and, for any t-ideal and k-filter $I$, we have $a \otimes b \in I$ iff  $a, b \in I$.

(iv). Follows from the fact that, for any prime bifilter $F$, we have $a \oplus b \in F$ iff $a \in F$ or $b \in F$ and, for any prime t-ideal and k-filter $I$, we have $a \oplus b \in I$ iff $a \in I$ or $b \in I$.

%Let us denote by $Pr \FF (\Al[B]) $ the family of prime bifilters of $\Al[B]$ and by  $Pr \IF (\Al[B]) $ the family of prime t-ideal and k-filters of $\Al[B]$. 

The previous items show that the family $\sigma[B] = \{ \sigma(a) : a \in B \}$ is  the universe of a
subbilattice of the bilattice $$\langle P( Pr \FF (\Al[B]) ), \cap, \cup \rangle \odot \langle P( Pr \IF (\Al[B]) ), \cap, \cup \rangle. $$ Injectivity of $\sigma$ follows from Proposition \ref{bifsep}. 


Notice that, if $\Al[B]$  has a negation, then there is an isomorphism between the set of all bifilters of $\Al[B]$ and the set of all t-ideals and k-filters of $\Al$. The isomorphism $i $ is defined as follows: for $F$ a bifilter, let us take $i(F) = \{ \neg a : a \in F \}$. So, in case the bilattice has a negation, we can define the isomorphism using bifilters only, as follows: 
\begin{align*}
\sigma^+(a) & = \{ X \subseteq B : X \textrm{ is a prime bifilter and } a \in X \}; \\
\sigma^-(a) & = \{ X \subseteq B : X \textrm{ is a prime bifilter and } \neg a \in X \}.
\end{align*}

Let us check that:

\begin{enumerate}[(i)]
\item $\sigma(a \land b)  = \langle \sigma^+(a) \cap \sigma^+(b), \sigma^-(a) \cup \sigma^-(b) \rangle$
\item  $\sigma(a \lor b)  = \langle \sigma^+(a) \cup \sigma^+(b), \sigma^-(a) \cap \sigma^-(b) \rangle$
\item $\sigma(a \otimes b)  = \langle \sigma^+(a) \cap \sigma^+(b), \sigma^-(a) \cap \sigma^-(b) \rangle$
\item $\sigma(a \oplus b)  = \langle \sigma^+(a) \cup \sigma^+(b), \sigma^-(a) \cup \sigma^-(b) \rangle$.
\item $\sigma (\neg a) = \langle \sigma^-(a), \sigma^+(a)  \rangle$.
\end{enumerate}

(i). Follows from the fact that, for any prime bifilter $F$, we have $a \land b \in F$ iff $a, b \in F$ and $\neg (a \land b) \in F$ iff $\neg a \lor \neg b \in F$ iff $\neg a \in F$ or $ \neg b \in F$.

(ii). For any prime bifilter $F$, we have $a \lor b \in F$ iff $a \in F$ or $b \in F$ and $\neg (a \lor b) \in F$ iff $\neg a \land \neg b \in F$ iff $\neg a, \neg b \in F$.

(iii). For any prime bifilter $F$, we have $a \otimes b \in F$ iff $a, b \in F$ and $\neg (a \otimes b) \in F$ iff $\neg a \otimes \neg b \in F$ iff $\neg a, \neg b \in F$.

(iv). For any prime bifilter $F$, we have $a \oplus b \in F$ iff $a \in F$ or $b \in F$ and $\neg (a \oplus b) \in F$ iff $\neg a \oplus \neg b \in F$ iff $\neg a \in F$ or $ \neg b \in F$.

(v). This last case is immediate.

So in this case the family $\sigma(B) = \{ \sigma(a) : a \in B \}$ is  the universe of a subbilattice of the bilattice $$\langle P(Pr \FF (\Al[B]) ), \cap, \cup \rangle \odot \langle P(Pr \FF (\Al[B])), \cap, \cup \rangle.$$ 
\end{proof}

\section{Bilattices with conflation}
\label{sec:confl}

Among the extensions of the bilattice language we have considered so far, a natural one is the one introduced by Fitting \cite{Fi94}, who defined a kind of dual negation operator, called \emph{conflation}. This gives rise to the following:


\begin{definition} \label{def:bilconf}
An algebra $\Al[B] =\la B, \land, \lor,
\otimes, \oplus, \neg,  \co \ra $ is a \emph{bilattice with conflation} if and only if  the reduct
$\left\langle B, \land, \lor,
\otimes, \oplus, \neg \right\rangle$ is a bilattice and the
\emph{conflation} $\co: B \longrightarrow B$ is an operation satisfying that for every $a,b \in B$,
\begin{enumerate}[]
 \item \quad \textbf{(con1)} \qquad if $a \leq_{k} b$,  then  $- b \leq_{k} - a$
 \item \quad \textbf{(con2)} \qquad  if $a \leq_{t} b$,  then  $- a \leq_{t} - b$ 
 \item \quad \textbf{(con3)} \qquad  $ a = - - a  $.
\end{enumerate}
We say that $\Al[B]$ is \emph{commutative} if it satisfies, for all $a \in B$, 
$$\neg \co  a = \co  \neg \: a.$$
\end{definition}

The following properties, analogue to those of negation, are easily proved:

\begin{proposition}[De Morgan laws]
\label{prop:dmc}
The following equations  hold in any bilattice with conflation: 
%$\Al[B] =\left\langle B, \land, \lor, \otimes, \oplus, \neg \right\rangle$:
\begin{align*}
 \label{eq:dmc}
\neg (x \otimes y) & \approx  - x \oplus - y     &&& - (x \oplus y)  & \approx - x \otimes - y \\
\neg (x \land y) & \approx - x \land - y &&&   - (x \lor y) & \approx - x \lor - y.
\end{align*} 
%
Moreover, if the bilattice is bounded, then $- \top = \bot$, $- \bot = \top$, $- \true = \true$ and
$- \false = \false$.
\end{proposition}


So, if a bilattice with conflation $\Al[B] =\left\langle B, \land, \lor, \otimes, \oplus, \neg \right\rangle$ is distributive, or at least the k-lattice of $\Al[B]$ is distributive, then the reduct $\la B, \otimes, \oplus,  - \ra$ is a De Morgan lattice. It is also easy to check that the four De Morgan laws imply that the conflation operator satisfies \textbf{(con1)} and \textbf{(con2)}.  Hence, the class of
bilattices with conflation
%, denoted by $\BLC$, 
is equationally axiomatizable. Adding the appropriate equations to a presentation of this class, we may define the varieties %$\IBLC$ and $\DBLC$ 
of interlaced (distributive) bilattices with conflation and of commutative (interlaced, distributive) bilattices with conflation.

Our next aim is to see how an analogue of our representation theorems can be proved for bilattices with conflation. To this end we introduce the following construction, also due to Fitting. %\cite{Fi94}. 
Let $\Al[L] = \la L, \sqcap, \sqcup, ' \ra$ be an algebra such that the reduct $ \la L, \sqcap, \sqcup \ra$ is a lattice and the operation $' : A \longrightarrow A$ satisfies, for all $a, b \in A$:
%\begin{enumerate}[(i)]
% \item if $a \leq  b$,  then  $ b' \leq a'$
% \item $ a = a''  $.
%\end{enumerate}
\begin{enumerate}[]
 \item \quad \textbf{(inv1)} \qquad if $a \leq  b$,  then  $ b' \leq a'$
 \item \quad \textbf{(inv2)} \qquad $ a = a''  $. 
\end{enumerate}
We call $\Al[L] = \la L, \sqcap, \sqcup, ' \ra$  a \emph{lattice with involution}.

Given a lattice with involution $\Al[L] = \la L, \sqcap, \sqcup, ' \ra$, we denote by $\Al[L] \odot \Al[L]$ the bilattice with conflation whose bilattice reduct is the usual product bilattice $ \la L, \sqcap, \sqcup \ra \odot \la L, \sqcap, \sqcup \ra$ and whose conflation is defined, for all $a, b \in L$, as $- \la a, b \ra = \la b', a' \ra$. It is easy to check that $\Al[L] \odot \Al[L]$ is indeed an interlaced bilattice with conflation. Moreover, it is commutative.

 Fitting \cite[Theorem 8.3]{Fi94} showed that, if $\Al[B]$ is a commutative distributive bilattice with conflation, then there is a De Morgan lattice $\Al[L]$ such that $\Al[B]$ is isomorphic to $\Al[L] \odot \Al[L]$. Using our Representation Theorem, it is easy to generalize this result to unbounded interlaced bilattices. We shall need the following:
 
\begin{lem} \label{lem:regconf}
Let $\Al[B]$ be a commutative interlaced bilattice with conflation. Then:
\begin{enumerate}[(i)]
 \item the set $\Reg(\Al[B])$ is closed under conflation,
 \item $\reg(a) = \co \reg (\neg \co a)$ for all $a \in B$.
\end{enumerate}
\end{lem}

\begin{proof}
(i). Using commutativity, we have that $a \in \Reg(\Al[B])$ implies $\neg \co a = \co \neg \: a = \co a $.

(ii). Using the Representation Theorem for interlaced bilattices, it is easy to check that, for all $a \in B$, it holds that
$$ \reg(a) = (a \land (a \oplus \neg a)) \otimes \neg (a \land (a \oplus \neg a)). $$ Now, applying De Morgan's laws and commutativity, we have
\begin{align*}
\co \reg (\neg \co a) 
& =  \co  ((\neg \co a \land (\neg \co a \oplus \neg \neg \co a)) \otimes \neg (\neg \co a \land (\neg \co a \oplus \neg \neg \co a)))      \\
& =  \co (\neg \co a \land (\neg \co a \oplus  \co a)) \oplus \co \neg (\neg \co a \land (\neg \co a \oplus  \co a))     \\
& =  (\co \neg \co a \land \co (\neg \co a \oplus  \co a)) \oplus  \neg \co (\neg \co a \land (\neg \co a \oplus  \co a))     \\
& =  ( \neg a \land (\co \neg \co a \otimes \co \co a)) \oplus  \neg  (\co \neg \co a \land \co (\neg \co a \oplus \co a)) \\
& =  ( \neg a \land (\neg a \otimes a)) \oplus  \neg  ( \neg a \land (\co \neg \co a \otimes \co \co a)) \\
& =  ( \neg a \land (\neg a \otimes a)) \oplus   ( \neg  \neg a \lor \neg (\neg a \otimes a)) \\
& =   \neg ( a \lor  \neg (\neg a \otimes a)) \oplus   (a \lor  (\neg \neg a \otimes \neg a)) \\
& =   \neg ( a \lor  ( a \otimes \neg a)) \oplus   (a \lor  (a \otimes \neg a)) \\
& = \reg (a). 
\end{align*}
\end{proof}

It is now easy to prove the following:

\begin{thm} [Representation, 3]
\label{thm:bl_conf}
Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus, \neg, \co \rangle$ be a commutative interlaced bilattice with conflation. Then $\Al[B]$ is isomorphic to the bilattice with conflation $\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle
  \odot \langle \Reg(\Al[B]), \otimes, \oplus, \co \rangle$, where $\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle$ is a lattice with involution.
\end{thm} 

\begin{proof}
Lemma \ref{lem:regconf} (i) implies that $\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle$ is a lattice with involution. Hence, we can construct the bilattice with conflation $\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle \odot \langle \Reg(\Al[B]), \otimes, \oplus, \co \rangle$ as defined above. We know that  $\langle B, \land, \lor, \otimes, \oplus, \neg \rangle$ is isomorphic to  $\la \Reg(\Al[B]), \otimes, \oplus \rangle \odot \la \Reg(\Al[B]), \otimes, \oplus \rangle$ via the map $f: B \longrightarrow \Reg(\Al[B]) \times \Reg(\Al[B])$ defined as $f(a) = \la \reg(a), \reg(\neg a) \ra$. We shall prove that $f$ also  preserves conflation, i.e.\ that $f(\co a) = \co f(a)$. Using Lemma \ref{lem:regconf} (ii) and commutativity, we have
%
\begin{align*}
f(\co a) & = \la \reg( \co a), \reg(\neg \co a) \ra\\
& = \la \co \reg( \neg \co \co a), \co \reg( \neg \co \neg \co a) \ra \\
& = \la \co \reg( \neg a), \co \reg( \neg  \neg \co \co a) \ra \\
& = \la \co \reg( \neg a), \co \reg( a) \ra \\
& =  \co (\la \reg(a), \reg(\neg a) \ra) \\
& = \co f(a).
\end{align*}
\end{proof}

The previous theorem immediately yields the following:

\begin{cor} 
\label{cor:distbl_conf}
Let $\Al[B] = \langle B, \land, \lor, \otimes, \oplus, \neg, \co \rangle$ be a commutative distributive bilattice with conflation. Then $\Al[B]$ is isomorphic to the bilattice with conflation $\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle
  \odot \langle \Reg(\Al[B]), \otimes, \oplus, \co \rangle$, where $\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle$ is a De Morgan lattice.
\end{cor} 

It may be interesting to note that, using Theorem~\ref{thm:bl_conf}, one can easily check that, for any commutative interlaced bilattice with conflation $\Al[L] \odot \Al[L]$% = \langle L \times L, \land, \lor, \otimes, \oplus, \neg, \co \rangle$
, 
where $\Al[L] = \la L, \sqcap, \sqcup, ' \ra$, there is an isomorphism $h$ between the two lattices with involution $ \langle L \times L, \land, \lor,  \neg \rangle$ and $ \langle L \times L, \otimes, \oplus, \co \rangle$ that may be defined, for all $a, b \in L$, as $h(\la a, b \ra) = \la a, b' \ra$.

We shall now give a characterization of the lattice of congruences of commutative interlaced bilattices with conflation, analogous to the one given for interlaced bilattices (see Proposition \ref{p:interbl_cong}). 

\begin{proposition} \label{p:blconf_cong}
Let  $\Al[B] = \langle B, \land, \lor, \otimes, \oplus, \neg, \co \rangle$ be a commutative interlaced bilattice with conflation. Then:
\begin{enumerate}[(i)]
 \item for all $\theta \in \Con (\Al[B] )$ and for all $a, b \in B$, it holds that $\la a, b \ra \in \theta $ if and only if $\la \reg(a), \reg(b) \ra \in \theta $ and  $\la \reg(\neg a), \reg(\neg b) \ra \in \theta $, 
 \item  $\la \Con (\Al[B] ), \subseteq \ra \cong \la \Con (\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle), \subseteq \ra$.
\end{enumerate}

\end{proposition}

\begin{proof}
(i). Recalling the  definition of regular element, it is easy to see that $\la a, b \ra \in \theta $ implies $\la \reg(a), \reg(b) \ra \in \theta $ and  $\la \reg(\neg a), \reg(\neg b) \ra \in \theta $. The converse is also easy, for, as we have observed, for all $a \in B$ we have
$$a = (\reg(a) \otimes (\reg(a) \lor \reg(\neg a))) \oplus (\reg(\neg a) \otimes (\reg(a) \land \reg(\neg a))).$$


(ii). We shall prove that the isomorphism is given by the map 
%
$$h: \Con (\Al[B] ) \longrightarrow \Con (\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle)$$
defined, for all $\theta \in  \Con (\Al[B])$, as $$h(\theta) = \theta \cap \Reg(\Al[B]) \times \Reg(\Al[B]).$$ 
 Clearly $h(\theta) \in \Con (\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle)$. It is also easy to see that $h$ is order-preserving, for $\theta_{1} \subseteq \theta_{2}$ implies $\theta_{1}   \cap \Reg(\Al[B]) \times \Reg(\Al[B]) \subseteq  \theta_{2}  \cap \Reg(\Al[B]) \times \Reg(\Al[B]) $. To see that it is order-reflecting, assume $h(\theta_{1}) \subseteq h(\theta_{2})$ and $\la a, b \ra \in \theta_{1}$. By (i) we have  $\la \reg(a), \reg(b) \ra \in \theta_{1} $ and  $\la \reg(\neg a), \reg(\neg b) \ra \in \theta_{1} $. Then the assumptions imply $\la \reg(a), \reg(b) \ra \in \theta_{2} $ and  $\la \reg(\neg a), \reg(\neg b) \ra \in \theta_{2} $, so, applying again (i), we obtain $\la a, b \ra \in \theta_{2}$. This proves that $h$ is an order embedding. To see that it is onto, we will show that its inverse is $$h^{-1}: \Con (\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle) \longrightarrow \Con (\Al[B] ) $$
defined, for all $\theta \in  \Con (\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle)$, as follows: 
$$ \la a, b \ra \in h^{-1}(\theta) \textrm{ iff }  \la \reg(a), \reg(b) \ra \in \theta \textrm{ and  } \la \reg(\neg a), \reg(\neg b) \ra \in \theta.$$
Clearly  $h^{-1}(\theta)$ is an equivalence relation. To see that $h^{-1}(\theta) \in \Con (\Al[B] ) $, recall that, by Proposition  \ref{prop:regular}, we have 
\begin{align*}
\reg(a \land b) & = \reg (a \otimes b) = \reg(a) \otimes \reg (b) \\
\reg(a \lor b) & = \reg (a \oplus b) = \reg(a) \oplus \reg (b).
\end{align*}
It is then clear that $ h^{-1}(\theta)$ is compatible with all the lattice operations of both orders, as well as with negation. As to conflation, assume $\la a, b \ra \in  h^{-1}(\theta)$, i.e.\ $\la \reg(a), \reg(b) \ra \in \theta$ and $\la \reg(\neg a), \reg(\neg b) \ra \in \theta$. From the latter, applying Lemma \ref{lem:regconf} (ii), we obtain
$\la \co \reg(\neg \co \neg a), \co \reg(\neg \co  \neg b) \ra \in \theta.$ Now, using commutativity and the fact that $\theta$ is compatible with conflation, we conclude that  $\la \reg( \co a), \reg( \co b) \ra \in \theta.$ A similar reasoning shows that $\la \reg(a), \reg(b) \ra \in \theta$ implies $\la \reg(\neg \co a), \reg(\neg \co b) \ra \in \theta$. Hence  $ \la \co a, \co b \ra \in  h^{-1}(\theta)$. Finally, it follows immediately from the definitions that $h(h^{-1}(\theta)) = \theta$.
\end{proof}

Note that the proof of item (i) of the previous proposition does not involve conflation: in fact this  property holds for any interlaced bilattice. Item (ii) allows us to obtain some information on the variety of commutative distributive bilattices with conflation, as shown by the following:

\begin{thm} 
\label{thm:varconf}
The variety of commutative distributive bilattices with conflation is generated by the bilattice with conflation $\Al[M_{4}] \odot \Al[M_{4}]$, where $\Al[M_{4}]$ denotes the four-element non-linear De Morgan lattice (i.e.\ the $\{\land, \lor, \neg \}$-reduct of the bilattice $\four$).
\end{thm}

\begin{proof}
By Proposition \ref{p:blconf_cong}, a commutative distributive bilattice with conflation $\Al[B]$ is subdirectly irreducible if and only if $\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle$ is subdirectly irreducible. Moreover, we have seen in Corollary \ref{cor:distbl_conf} that $\la \Reg(\Al[B]), \otimes, \oplus, \co \rangle$ is a De Morgan lattice. It is known (see for instance \cite{F97}) that  the only subdirectly irreducible De Morgan lattices are $\Al[M_{4}]$, the two-element chain $\Al[B_{2}]$ and the three-element chain $\Al[K_{3}]$. Hence, the only subdirectly irreducible commutative distributive bilattices with conflation are $\Al[M_{4}]\odot \Al[M_{4}]$, $\Al[K_{3}] \odot \Al[K_{3}]$ and $\Al[B_{2}] \odot \Al[B_{2}]$. Therefore these algebras generate the variety of commutative distributive bilattices with conflation, and indeed  $\Al[M_{4}]\odot \Al[M_{4}]$ alone generates it, for it is easy to see that $\Al[K_{3}] \odot \Al[K_{3}]$ and $\Al[B_{2}] \odot \Al[B_{2}]$ are isomorphic to subalgebras of $\Al[M_{4}]\odot \Al[M_{4}]$.
\end{proof}
 
An easy consequence of the previous theorem is that, as it happens with De Morgan lattices, the variety of commutative distributive bilattices with conflation has exactly two proper subvarieties, namely the variety generated by $\Al[K_{3}] \odot \Al[K_{3}]$, which we call of \emph{Kleene bilattices with conflation} ($\KB$) and the one generated by $\Al[B_{2}] \odot \Al[B_{2}]$, which we call (following \cite{ArAv96}) of \emph{classical bilattices with conflation} ($\CB$). It is also easy to provide an equational presentation for these varieties:

\begin{thm} 
\label{thm:confklee}
The variety $\KB$ is axiomatized by the identities defining commutative distributive bilattices with conflation plus either of the following ones:
\begin{enumerate}[(i)]
 \item \qquad $(x \land \neg \co x) \land (y \lor \neg \co y) \approx (x \land \neg \co x)$ 
 \item \qquad $(x \otimes \neg \co x) \otimes (y \oplus \neg \co y) \approx (x \otimes \neg \co x).$
\end{enumerate}
%
%\begin{align*}
%  (x \land \neg \co x) \land (y \lor \neg \co y) & \approx (x \land \neg \co x)    && \textrm{(i)}   \\
%   (x \otimes \neg \co x) \otimes (y \oplus \neg \co y)  &  \approx (x \otimes \neg \co x) && \textrm{(ii)}  
%\end{align*}
\end{thm}

\begin{proof}
It is known (see for instance \cite{F97}) that the variety of Kleene lattices $\Al[L] = \la L, \sqcap, \sqcup, ' \ra$ is generated by  $\Al[K_{3}]$ and axiomatized by the identities for De Morgan lattices plus the following: $ (x \sqcap x') \sqcap (y \sqcup  y') \approx (x \sqcap x')$. Using Corollary~\ref{cor:distbl_conf}, it is easy to check that if a commutative distributive bilattice with conflation $\Al[L] \odot \Al[L]$ satisfies (i) or (ii), then $\Al[L] = \la L, \sqcap, \sqcup, ' \ra$ satisfies  $ (x \sqcap x') \sqcap (y \sqcup  y') \approx (x \sqcap x')$. For instance, using (i), we have that for any $a_{1}, a_{2}, b_{1}, b_{2} \in L$:
%
\begin{align*}
    \la a_{1}, a_{2} \ra \land \neg \co \la a_{1}, a_{2} \ra & = \la a_{1}, a_{2} \ra \land  \la a_{1}', a_{2}' \ra  \\
    & = \la a_{1} \sqcap a_{1}', a_{2} \sqcup a_{2}' \ra   \\
    &  \leq_{t} \la b_{1} \sqcup b_{1}', b_{2} \sqcap b_{2}'   \ra \\
   & = \la b_{1}, b_{2} \ra \lor  \la b_{1}', b_{2}' \ra  \\
  & = \la b_{1}, b_{2} \ra \lor \neg \co \la b_{1}, b_{2} \ra.
\end{align*}
That is, $a_{1} \sqcap a_{1}' \leq b_{1} \sqcup b_{1}' $ and $a_{2} \sqcup a_{2}' \geq  b_{2} \sqcap b_{2}'  $. Hence $\Al[L]$ is a Kleene lattice. Conversely, for any Kleene lattice $\Al[L]$, the bilattice with conflation $\Al[L] \odot \Al[L]$ will satisfy (i) and (ii). 
\end{proof}

\begin{thm} 
\label{thm:confbool}
The variety $\CB$  is axiomatized by the identities defining commutative distributive bilattices with conflation plus any of the following ones:
\begin{enumerate}[(i)]
 \item \qquad $x \land (y \lor \neg \co y) \approx x$ 
 \item \qquad $x \otimes (y \oplus \neg \co y) \approx x$
 \item \qquad $x \lor (y \land \neg \co y) \approx x$ 
  \item \qquad  $x \oplus (y \otimes \neg \co y) \approx x.$ 
\end{enumerate}
\end{thm}

\begin{proof}
Similar to the proof of the previous theorem. The variety of Boolean lattices $\Al[L] = \la L, \sqcap, \sqcup, ' \ra$ is generated by  $\Al[B_{2}]$ and axiomatized by the identities for De Morgan lattices plus either of the following: $ x \sqcap (y \sqcup  y') \approx x $ or $ x \sqcup (y \sqcap  y') \approx x $. Using Corollary~\ref{cor:distbl_conf}, it is easy to check that if a commutative distributive bilattice with conflation $\Al[L] \odot \Al[L]$ satisfies any of the equations (i) to (iv), then $\Al[L] = \la L, \sqcap, \sqcup, ' \ra$ satisfies  $ x \sqcap (y \sqcup  y') \approx x $ and $ x \sqcup (y \sqcap  y') \approx x $, hence is a Boolean lattice. Conversely, for any Boolean lattice $\Al[L]$, the bilattice with conflation $\Al[L] \odot \Al[L]$ will satisfy (i) to (iv). 
\end{proof}

 


%\bibliography{logalg}{}
%\bibliographystyle{plain}

%\end{document} 


==> dedica.tex <==
\thispagestyle{plain}
\mbox{}
\vspace{2in}
\begin{center}
{\em to me \\ \ \\
who did all the work on this}
%\footnote{The dedication is optional}
\end{center}

